Molecular Algebraic Geometry: Electronic Structure of H$_3^+$ as Algebraic Variety

In this article, we demonstrate the restricted Hartree-Fock electronic structure computation of the molecule $H_3^+$ through computational algebra. We approximate the Hartree-Fock total energy by a polynomial composed of LCAO coefficients and atomic distances so that the minimum is determined by a set of polynomial equations. We get the roots of this set of equations through the techniques of computational algebraic geometry, namely, the Gr\"obner basis and primary ideal decomposition. This treatment enables us to describe the electronic structures as algebraic varieties in terms of polynomials.

==> SCRAPINGOUT.tex <==
option(noredefine);LIB "solve.lib";option(redSB);
ring r=0,(x, y, z, e),dp;
short=0;
poly OBJ=-20000*e*x**2 - 22288*e*x*y - 22288*e*x*z - 20000*e*y**2 - 22288*e*y*z - 20000*e*z**2 + 20000*e + 7746*x**4 + 14316*x**3*y + 14316*x**3*z + 18392*x**2*y**2 + 26758*x**2*y*z + 18392*x**2*z**2 - 31781*x**2 + 14316*x*y**3 + 26758*x*y**2*z + 26758*x*y*z**2 - 44637*x*y + 14316*x*z**3 - 44637*x*z + 7746*y**4 + 14316*y**3*z + 18392*y**2*z**2 - 31781*y**2 + 14316*y*z**3 - 44637*y*z + 7746*z**4 - 31781*z**2 + 17639;
list diffs;
for(int i=1;i<=nvars(r); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}
ideal I=0;
for(int i=1;i<=nvars(r); i=i+1){I=I+diff(OBJ,var(i));}
print(I);ideal SI=std(I);
write(":w save_std_dp.txt",SI);
print(SI);ring s=0,(x, y, z, e),lp;
setring s;short=0;
ideal j=fglm(r,SI);
 j;
write(":w save_std.txt",j);
LIB "triang.lib";
list TRJ=triangM(j);
write(":w save_t.txt",TRJ);
for (int index=1; index<=size(TRJ); index=index+1)
{
 setring s;
 print("+++++++++++++");
 print("index");
 print(index);
 print(size(TRJ));
 ideal TR=TRJ[index];
 print(TR);
 def R=triang_solve(TR,50);
 setring R;short=0;rlist; 
 string name=":w trlist"+string(index)+".txt";
 string sr=print(rlist,"%s");
 write(name,sr);
 setring s;
}

setring s;	
LIB "rootsmr.lib";
ideal b = qbase(j);
write(":w save_qbase.txt",b);

list matmults;
for (int i=1;i<=nvars(r); i=i+1){
poly f=var(i);
matrix m = matmult(f,b,j);
//print(f);
//m;
matmults=insert(matmults,m,size(matmults));
}
matrix mx = matmult(x,b,j);
matrix my = matmult(y,b,j);
matrix mz = matmult(z,b,j);
matrix me = matmult(e,b,j);
write(":w save_matmult.txt",matmults);
write(":w save_mx.txt",string(mx));
write(":w save_my.txt",string(my));
write(":w save_mz.txt",string(mz));
write(":w save_me.txt",string(me));
size(matmults);
mx;
my;
mz;
me;


def R=triang_solve(j,50);
setring R;short=0;rlist;
poly OBJ=fetch(r,OBJ);
ideal I=fetch(r,I);
OBJ;
list subste;
for (i=1;i<=size(rlist);i=i+1){
list substv;

poly OBJ2=OBJ;
for (int k=1; k<=nvars(R); k=k+1)
{
 OBJ2=subst(OBJ2,var(k), rlist[i][k]);
}
substv=insert(substv,OBJ2);

for (int l=1;l<=size(I);l=l+1)
{
 poly OBJ2=I[l];
 for (int k=1; k<=nvars(R); k=k+1)
 {
  OBJ2=subst(OBJ2,var(k), rlist[i][k]);
 }
 substv=insert(substv,OBJ2,size(substv));
}
print("substv");print(substv);
subste=insert(subste,substv,size(subste));
}
write(":w save_i.txt",rlist);
write(":w save_e.txt",subste);
print("subste");
print(subste);

setring r;
ideal J=x-y,y-z;
ideal I_J=quotient(SI,J);
I_J;
ideal stdI_J=std(I_J);
stdI_J;
ideal JXYZ=x*y*z;
ideal IJ_JXYZ=quotient(I_J,JXYZ);
ideal stdIJ_JXYZ=std(IJ_JXYZ);
setring s;
//ideal j1=fglm(r,stdIJ_XYZ);
//j1;


//stdIJ_JXYZ;

setring s;

ideal Q1=fglm(r,stdI_J);
Q1;
TRJ=triangM(Q1);
write(":w save_TQ1.txt",TRJ);
for (int index=1; index<=size(TRJ); index=index+1)
{
 setring s;
 ideal TR=TRJ[index];
 print(TR);
 def R=triang_solve(TR,50);
 setring R;rlist; setring s;
}
ideal Q2=fglm(r,stdIJ_JXYZ);
Q2;
TRJ=triangM(Q2);
TRJ;
write(":w save_TQ2.txt",TRJ);
for (int index=1; index<=size(TRJ); index=index+1)
{
 setring s;
 ideal TR=TRJ[index];
 print(TR);
 def R=triang_solve(TR,50);
 setring R;rlist; setring s;
}

setring r;
ideal JT=x-y,z+2*x;
ideal I_JT=quotient(I,JT);
I_JT;
SI;


==> VIRTUAL-ORBITALS.tex <==
#!/usr/bin/env python
# coding: utf-8

# These Python programs compute the electronic structure of H3+ in the equilateral triangle. 
# 
# The atoms are indexed by A, B, and C, or a, b, and c.
# The STO-3G are determined by the parameters ZETA, COEFF, and EXPON. 
# 
# (1) SZ-SIM-H3P-RHF
#       For RHF computation.  
#       The variables (x,y,z) : the LCAO coefficients of 1s orbitals on the vertices.
#       The variable e : the orbital energy
#       The variable R: the length of the edges, fixed at a positive number.
# 
# (2) SZ-SIM-H3P-UHF
#       For UHF computation.  
#       The variables (x,y,z) : the LCAO coefficients of 1s orbitals on the vertices, for spin alpha
#       The variables e : the orbital energy, for spin alpha
#       The variables (u,v,w) : the LCAO coefficients of 1s orbitals on the vertices, for spin beta
#       The variables f : the orbital energy, for spin beta
#       The variable R: the length of the edges, fixed at a positive number.
# 
# (3) SZ-SIM-H3P-RHF-DeterminR, SZ-SIM-H3P-RHF-DeterminR-Version2
#       The variables (x,x,x) : the LCAO coefficients of 1s orbitals on the vertices.
#       The variable e : the orbital energy
#       The variable R: the length of the edges, to be optimized as well as other variables.

# In[ ]:


#!/usr/bin/env python
# coding: utf-8

#
#  SUNDRY DEFINITIONS OF WORKING VARIABLES.
#
import networkx as nx

IG=nx.DiGraph() 
from sympy import symbols, Function,expand,sqrt
import numpy as np
import copy
from itertools import combinations_with_replacement, permutations,product

S12,T11,T12,T22,V11A,V12A,V22A,V11B,V12B,V22B,V1111,V2111,V2121,V2211,V2221,V2222=[0 for _ in range(16)]

S=[[0 for _ in range(2)] for _ in range(2)]
X=[[0 for _ in range(2)] for _  in range(2)]
NM=[[0 for _ in range(2)] for _  in range(2)]
XT=[[0 for _ in range(2)] for _ in  range(2)]
H=[[0 for _ in range(2)] for _ in  range(2)]
F=[[0 for _ in range(2)] for _ in  range(2)]
P=[[0 for _ in range(2)] for _  in range(2)]
G=[[0 for _ in range(2)] for _ in  range(2)]
F2=[[0 for _ in range(2)] for _ in  range(2)]
P2=[[0 for _ in range(2)] for _  in range(2)]
G2=[[0 for _ in range(2)] for _ in  range(2)]

C=[[0 for _ in range(2)] for _ in  range(2)]
FPRIME=[[0 for _ in range(2)] for _  in range(2)]
CPRIME=[[0 for _ in range(2)] for _  in range(2)]
P=[[0 for _ in range(2)] for _  in range(2)]
ODLPP=[[0 for _ in range(2)] for _  in range(2)]
E=[[0 for _ in range(2)] for _  in range(2)]
TT=[[[[0 for _ in range(2)] for _  in range(2)] for _ in range(2)] for _ in range(2)]

IOP=2
N=3
ZETA1=2.0925
ZETA2=1.24
ZA=2.0
ZB=1.0
#
#  Atomic distance R
#
R=symbols("R",positive=True)
#
#  Wavefunction (x,y) for alpha spin
#  Wavefunction (v,w) for beta spin
#
v, w = symbols("v w")
x, y = symbols("x y")


#
# In the following, we compute the atomic orbital integrals by the Gaussian orbital 
#  exp(-A*|r-RA|^2),exp(-A*|B-RB|^2),exp(-C*|r-RC|^2),exp(-D*|r-RD|^2)
#

import sympy as sympy
from sympy import symbols, Function,expand,core,sqrt
import numpy as np


def F0(ARG):
#
# BOYS F0 FUNCTIOM
#
    PI = sympy.pi
    if  type(ARG)==float and ARG < 1.0e-6:
        return 1 -ARG/3.
    if  type(ARG)==sympy.core.numbers.Zero and ARG < 1.0e-6:
        return 1 -ARG/3.
    else:
        #print("F0:ARG",ARG)
        if ARG!=sympy.S.Zero:
            return sympy.sqrt(PI/ARG)*sympy.erf(sqrt(ARG))/2
        else:
            return 1
    
def S000000(A,B,RA,RB):
#
#   OVERLAP INTEGRAL between exp(-A*|r-RA|^2) and exp(-B*|r-RB|^2)
#
    RAB2=sum([(c1-c2)**2 for c1,c2 in zip(RA,RB)])
    PI=np.pi
    print(A,B,RAB2,(PI/(A+B))**1.5)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def getS(A,B,RAB2):
#
# Calculates the overlap matrix between exp(-A*|r-RA|^2) and exp(-A*|B-RB|^2)
# WHEN RAB2=|RA-RB|^2
#
    PI=np.pi
    print(A,B,RAB2,(PI/(A+B))**1.5)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def K000000(A,B,RA,RB):
    RAB2=sum([(c1-c2)**2 for c1,c2 in zip(RA,RB)])
    PI=np.pi
    return A*B/(A+B)*(3.0-2.0*A*B*RAB2/(A+B))*(PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))   

def getT(A,B,RAB2):
#
# Calculates the kinetic energy
#  between exp(-A*|r-RA|^2) and exp(-B*|r-RB|^2)
# WHEN RAB2=|RA-RB|^2
#
    PI=np.pi
    return A*B/(A+B)*(3.0-2.0*A*B*RAB2/(A+B))*(PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def V(A,B,RAB2,RCP2,ZC):
#
#  CALCULATES UN-NORMALIZED NUCLEAR ATTRACTION INTEGRALS
#
    PI=np.pi
    V=2.0*PI/(A+B)*F0((A+B)*RCP2)*sympy.exp(-A*B*RAB2/(A+B))
    return -V*ZC

def TWOE(A,B,C,D,RAB2,RCD2,RPQ2):
#
# CALCULATES TWO-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
# A,B,C,D ARE THE EXPONENTS ALPHA, BETA, ETC.
# RAB2 EQUALS SQUARED DISTANCE BETWEEN CENTER A AND CENTER B, ETC.
#
# The integrand is the product of those functions.
#   exp(-A*|r1-RA|^2),exp(-B*|r1-RB|^2),1/|r1-r2|, exp(-C*|r2-RC|^2),exp(-D*|r2-RD|^2)
# when RB=RA and RD=RC.
#
#
    PI=np.pi
    return 2.0*(PI**2.5)/((A+B)*(C+D)*np.sqrt(A+B+C+D))*F0((A+B)*(C+D)*RPQ2/(A+B+C+D))*sympy.exp(-A*B*RAB2/(A+B)-C*D*RCD2/(C+D))

    
def BOYS(N,X):
#
#  BOYS FUNCTION F_N(X)
#
    if N==0:
        return F0(X)
    else:
        Z=Symbol("Z")
        f=F0(Z)
        for _ in range(N):
            f=f.diff(Z)*(-1)
        return f.subs(Z,X)
    
def KXYZAB(a,b,RA,RB):
    mu=a*b/(a+b)
    RAB=[(c1-c2)**2 for c1,c2 in zip(RA,RB)]
    RAB2=sum(RAB)
    return sympy.exp(-mu*RAB2)

def T0000(a,b,c,d,RA,RB,RC,RD):
#
# CALCULATES TWO-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
# a,b,c,d ARE THE EXPONENTS ALPHA, BETA, ETC.
# RAB2 EQUALS SQUARED DISTANCE BETWEEN CENTER A AND CENTER B, ETC.
#
# The integrand is the product of those functions.
#   exp(-a*|r1-RA|^2),exp(-b*|r1-RB|^2),1/|r1-r2|, exp(-c*|r2-RC|^2),exp(-d*|r2-RD|^2)
#
#
    def MF0(ARG):
    #
    # BOYS F0 FUNCTIOM
    #
        PI = sympy.pi
        if  type(ARG)==float and ARG < 1.0e-6:
            return 1 -ARG/3.
        if  type(ARG)==sympy.core.numbers.Zero and ARG < 1.0e-6:
            return 1 -ARG/3.
        else:
            #print("F0:ARG",ARG)
            if ARG!=sympy.S.Zero:
                return sympy.sqrt(PI/ARG)*sympy.erf(sqrt(ARG))/2
            else:
                return 1
    p=a+b
    q=c+d
    RP=[(a*c1+b*c2)/(a+b) for c1,c2 in zip(RA,RB)]
    RQ=[(c*c1+d*c2)/(c+d) for c1,c2 in zip(RC,RD)]
    alpha=p*q/(p+q)
    PI=sympy.pi
    RPQ=[(c1-c2)**2 for c1,c2 in zip(RP,RQ)]
    RPQ2=sum(RPQ)
    return 2*PI**(2.5)/p/q/sympy.sqrt(p+q)*KXYZAB(a,b,RA,RB)*KXYZAB(c,d,RC,RD)*MF0(alpha*RPQ2)

def V000000(a,b,RA,RB,RC):
#
# CALCULATES ONE-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
#
#  The integrand is the product of those functions.
#   exp(-a*|r-RA|^2),exp(-b*|r-RB|^2),1/|r-RC|
#  
    p=a+b
    PI=sympy.pi
    RP=[(a*c1+b*c2)/(a+b) for c1,c2 in zip(RA,RB)]
    RPC=[(c1-c2)**2 for c1,c2 in zip(RP,RC)]
    RPC2=sum(RPC)
    return 2*PI/p*KXYZAB(a,b,RA,RB)*BOYS(0,p*RPC2)

def TN0000(N,a,b,c,d,RA,RB,RC,RD):
#
#  This function is the simplest case of the so-Called auxilary function THETA(N;000 000 000 000)
#  in Obara-Saika Schme for two-electron integrals.
#
    if N<0:
        return 0
    p=a+b
    q=c+d
    RP=[(a*c1+b*c2)/(a+b) for c1,c2 in zip(RA,RB)]
    RQ=[(c*c1+d*c2)/(c+d) for c1,c2 in zip(RC,RD)]
    alpha=p*q/(p+q)
    PI=sympy.pi
    RPQ=[(c1-c2)**2 for c1,c2 in zip(RP,RQ)]
    RPQ2=sum(RPQ)
    return 2*PI**(2.5)/p/q/sympy.sqrt(p+q)*KXYZAB(a,b,RA,RB)*KXYZAB(c,d,RC,RD)*BOYS(N,alpha*RPQ2)


#
#  TEST
#
AX,AY,AZ,BX,BY,BZ,CX,CY,CZ,DX,DY,DZ=symbols("AX AY AZ BX BY BZ CX CY CZ DX DY DZ")
z1,z2,z3,z4=symbols("z1 z2 z3 z4")
f=T0000(z1,z2,z3,z4,[AX,AY,AZ],[BX,BY,BZ],[CX,CY,CZ],[DX,DY,DZ])
print(f)


#
# TEST
#
((S000000(z1,z2,[AX,AY,AZ],[BX,BY,BZ]).diff(AX)).diff(AX)).subs([(BX,AX),(BY,AY),(BZ,AZ)])


# #
# # PERFORMANCE TEST CONCERNING DIFFERENTIATION (TO GENERATE TWO-ELECTRON INTERGRALS OF P-ORBITALS)
# #
# #
# import time,random
# ALL=[]
# for va in [AX,AY,AZ]:
#     for vb in [BX,BY,BZ]:
#         for vc in [CX,CY,CZ]:
#             for vd in [DX,DY,DZ]:
#                 z1,z2,z3,z4=symbols("z1 z2 z3 z4")
#                 z1,z2,z3,z4=[random.random() for _ in range(4)]
#                 #z1,z2,z3,z4=[z1,z2,random.random(),random.random()]
#                 f0=T0000(z1,z2,z3,z4,[AX,AY,AZ],[BX,BY,BZ],[CX,CY,CZ],[DX,DY,DZ])
#                 #print(f)
#                 #print(va,vb,vc,vd)
#                 start=time.time()
# 
#                 f1=f0.diff(va)
#                 
#                 f2=f1.diff(vb)
#                 f3=f2.diff(vc)
#                 f4=f3.diff(vd)
#                 
#                 end=time.time()
# 
#                 print("time=",end-start)
#                 ALL.append([f0,f1,f2,f3,f4])




from sympy import Function, Symbol
TN=Function("TN0000")
UNDEF=Function("UNDEF")

from sympy import Number
class FMA(Function):
    """
    FMA(x, y, z) = x*y + z
    """
    @classmethod
    def eval(cls, x, y, z):
        # Number is the base class of Integer, Rational, and Float
        if all(isinstance(i, Number) for i in [x, y, z]):
           return x*y + z
    def doit(self, deep=True, **hints):
        x, y, z = self.args
        # Recursively call doit() on the args whenever deep=True.
        # Be sure to pass deep=True and **hints through here.
        if deep:
            x = x.doit(deep=deep, **hints)
            y = y.doit(deep=deep, **hints)
            z = z.doit(deep=deep, **hints)
        return x*y + z
    
    


# # Obara-Saika Scheme for Two-electron integrals



#
# We prepare dummy expressions for THE FUNCTIONS TN0000(N,a,b,c,d,RA,RB,RC,RD): TNS[0],TNS[1],...., WHICH SHALL BE USED LATER
#  THEY ARE AUXILLARY INTEGRALS, AND IF N=0 , THEY ARE THE TWO-ELECTRON INTGRALS.
#

TNSTRING=''
for i in range(11):
    TNSTRING+= 'TN'+str(i)+' '
TNS=symbols(TNSTRING)
def TN(N):
    return TNS[N]




#
#  INITIALIZATION OF OBARA-SAIKA
#
#INTEGRALALL=dict()
#for i in range(11):
#    INTEGRALALL[(i,0,0,0,0,0,0,0,0,0,0,0,0)]=TN(i)
    
IG=nx.DiGraph() 




#
#  EACH NUCLEI IS STATIONED IN THE 3D CARTESIAN SPACE:r=(x,y,z)
#  THE COORDINATES ARE REPRESENTED AS RA=(XA,YA,ZB)
#  THE DIFFERENCE ARE REPRESENTED BY XPA=XP-XA, YPQ=YP-YQ, ZAB=ZA-AB, AND SO ON.
#
#  WE START FROM SPHERICAL GAUSSIAN FUNCTIONS : (a,RA)=exp(-a|r-RA|^2),exp(-b|r-RB|^2),exp(-c|r-RC|^2),exp(-d|r-rB|^2).
#
#
#
XPA, XPQ, XCD, XAB=symbols("XPA XPQ XCD XAB")
YPA, YPQ,YCD, YAB=symbols("YPA YPQ YCD YAB")
ZPA, ZPQ, ZCD, ZAB=symbols("ZPA ZPQ ZCD ZAB")
XQC, YQC, ZQC=symbols("XQC YQC ZQC")
#
#
#  [(a,RA;r1),(b,Rb;r1)| 1/|r1-r2| | (c,Rd);r2,(d,RD;r2)] 
#
#
#  We put p=a*b/(a+b);q=c*d/(c+d); alpha=p*q/(p+q).
#  Provisionally p,q are left as they are without substitution.
#  At the end of the computation, we have to replace them.
#
a,b,c,d=symbols("a b c d")
p,q=symbols("p q")
alpha=symbols("alpha")

#
#  We compute the integrals using general Cartesian Gaussian functions:
#   (x-XA)^i (y-YA)^j (z-ZA)^j exp(-a|r-RA|^2)
#
#  VIZ.
#   [(i1,j1,k1,a,RA),(i2,j2,k2,b,RB)|1/|r1-r2||(i3,j3,k3,d,RC),(i4,j4,k4,d,RD)]
#
#  For brevity, we write:
#   i=(i1,i2,i3), j=(j1,j2,j3), k=(k1,k2,k3),
# 
#  To compute the auxillary integdals T(N,i,j,k,l) we lift from T(N,i=0.j=0,k=0,z=0)
#  WHEN N=0 THEY GIVE THE TWO-ELECTRON INTEGRALS; OBARA-SAIKA RECURSION USES THEM WITH N>=1.
#
#  BY VERTICAL RECUSION IN OBARA-SAIKA, WE COMPUTE 
#  (N: i+1 0 0 0 ) from (N: i 0 0 0) , (N+1 i 0 0 0) , (N i-1 0 0 0), (N+1 i 0 0 0)
#
#  WHERE i+1 is the every possible move from (i1,i2,i3) by adding one or zero to each of (i1,i2,i3), 
#  except zero-move. 
#
#  THE FOLLOWING FUNCTION LIFTS UP IN D=X/Y/Z DIRECTIONS AND COMPUTES THE INTGRALS.

def VERTICAL(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,INFO=0):
    alpha=p*q/(p+q)
    
    if D=="X":
        assert (j1==j2==j3==k1==k2==k3==l1==l2==l3==0),print(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,"X")
        #print("X")
        key0=(N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key1=(N+1,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key2=(N,i1-1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key3=(N+1,i1-1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        keyn=(N,i1+1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        i_d,k_d=i1,k1
        #print(keyn)
        DPA=XPA
        DPQ=XPQ
    if D=="Y":
        #print("Y")
        assert (j1==j2==j3==k1==k2==k3==l1==l2==l3==0),print(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,"X")
        key0=(N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key1=(N+1,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key2=(N,i1,i2-1,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key3=(N+1,i1,i2-1,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        keyn=(N,i1,i2+1,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        i_d,k_d=i2,k2
        #print(keyn)
        DPA=YPA
        DPQ=YPQ
    if D=="Z":
        assert (j1==j2==j3==k1==k2==k3==l1==l2==l3==0),print(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,"X")
        #print("Z")
        key0=(N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key1=(N+1,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key2=(N,i1,i2,i3-1,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key3=(N+1,i1,i2,i3-1,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        keyn=(N,i1,i2,i3+1,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        i_d,k_d=i3,k3
        #print(keyn)
        DPA=ZPA
        DPQ=ZPQ
    if None!=integrals_all.get(keyn):
        return
    
    data0=integrals_all.get(key0)
    data1=integrals_all.get(key1)
    data2=integrals_all.get(key2)
    data3=integrals_all.get(key3)
    #print(key0,key1,key2,key3)
    #print(data0,data1,data2,data3)
    nx.add_star(IG, [keyn,key0, key1, key2, key3])
    if min(list(key2))<0:
        data2=0
        integrals_all[key2]=0
    if min(list(key3))<0:
        data3=0
        integrals_all[key3]=0
    if data0==None:
        #print("data 0 requested")
        requested_keys[key0]=key0
    if data1==None:
        #print("data 1 requested")
        requested_keys[key1]=key1
    if data2==None:
        #print("data 2 requested")
        requested_keys[key2]=key2
    if data3==None:
        #print("data 3 requested")
        requested_keys[key3]=key3
    #print(requested_keys.keys())
    if data0!=None and data1!=None and data2!=None and data3!=None:
        if (INFO==1):
            print(keyn,"WRITTEN")
        integrals_all[keyn]= DPA*data0-alpha/p*DPQ*data1+i_d/2/p*(data2-alpha/p*data3)
    else:
        if (INFO==1):
            print(keyn,"NOT WRITTEN")
            print(key0,key1,key2,key3)
            print(data0,data1,data2,data3)
        else:
            pass
    return
    
#
#  The indices of the integrals which are required, but has not yet been computed.
#
requested_keys=dict()
        
#
#  The dictionary of computed integrals
#
integrals_all=dict()
for i in range(11):
    integrals_all[(i,0,0,0,0,0,0,0,0,0,0,0,0)]=TN(i)        


# V1111=0.0
# V2111=0.0
# V2121=0.0
# V2211=0.0
# V2221=0.0
# V2222=0.0
# N=3
# COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
# EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
# AtomA=[0,0,0]
# R_length=0.9/0.529177
# AtomB=[R_length,0,0]
# ZETA1=2.0925
# ZETA2=1.24
# ZETA1=ZETA2
# A1=[0]*N
# D1=[0]*N
# A2=[0]*N
# D2=[0]*N
# PI=np.pi
# for i in range(N):
#     #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
#     A1[i]=EXPON[N-1][i]*ZETA1**2
#     D1[i]=COEF[N-1][i]*((2.0*A1[i]/PI)**0.75)
#     A2[i]=EXPON[N-1][i]*(ZETA2**2)
#     D2[i]=COEF[N-1][i]*((2.0*A2[i]/PI)**0.75)
# for I in range(N):
#     for J in range(N):
#         for K in range(N):
#             for L in range(N):
#                 RAP=A2[I]*R/(A2[I]+A1[J])
#                 RBP=R-RAP
#                 RAQ=A2[K]*R/(A2[K]+A1[L])
#                 RBQ=R-RAQ
#                 RPQ=RAP-RAQ
#                 RAP2=RAP*RAP
#                 RBP2=RBP*RBP
#                 RAQ2=RAQ*RAQ
#                 RBQ2=RBQ*RBQ
#                 RPQ2=RPQ*RPQ
#                 """
#                 V1111=V1111+TWOE(A1[I],A1[J],A1[K],A1[L],0.0,0.0,0.0)*D1[I]*D1[J]*D1[K]*D1[L]
#                 V2111=V2111+TWOE(A2[I],A1[J],A1[K],A1[L],R2,0.0,RAP2)*D2[I]*D1[J]*D1[K]*D1[L]
#                 V2121=V2121+TWOE(A2[I],A1[J],A2[K],A1[L],R2,R2,RPQ2)*D2[I]*D1[J]*D2[K]*D1[L]
#                 V2211=V2211+TWOE(A2[I],A2[J],A1[K],A1[L],0.0,0.0,R2)*D2[I]*D2[J]*D1[K]*D1[L]
#                 V2221=V2221+TWOE(A2[I],A2[J],A2[K],A1[L],0.0,R2,RBQ2)*D2[I]*D2[J]*D2[K]*D1[L]
#                 V2222=V2222+TWOE(A2[I],A2[J],A2[K],A2[L],0.0,0.0,0.0)*D2[I]*D2[J]*D2[K]*D2[L]
#                 """
#                 ca=A1[I]
#                 cb=A1[J]
#                 cc=A1[K]
#                 cd=A1[L]
#                 """
#                 V1111=V1111+T0000(A1[I],A1[J],A1[K],A1[L],AtomA,AtomA,AtomA,AtomA)*D1[I]*D1[J]*D1[K]*D1[L]
#                 V2111=V2111+T0000(A2[I],A1[J],A1[K],A1[L],AtomB,AtomA,AtomA,AtomA)*D2[I]*D1[J]*D1[K]*D1[L]
#                 V2121=V2121+T0000(A2[I],A1[J],A2[K],A1[L],AtomB,AtomA,AtomB,AtomA)*D2[I]*D1[J]*D2[K]*D1[L]
#                 V2211=V2211+T0000(A2[I],A2[J],A1[K],A1[L],AtomB,AtomB,AtomA,AtomA)*D2[I]*D2[J]*D1[K]*D1[L]
#                 V2221=V2221+T0000(A2[I],A2[J],A2[K],A1[L],AtomB,AtomB,AtomB,AtomA)*D2[I]*D2[J]*D2[K]*D1[L]
#                 V2222=V2222+T0000(A2[I],A2[J],A2[K],A2[L],AtomB,AtomB,AtomB,AtomB)*D2[I]*D2[J]*D2[K]*D2[L]
#                 """
#                 V1111=V1111+T0000(ca,cb,cc,cd,AtomA,AtomA,AtomA,AtomA)*D1[I]*D1[J]*D1[K]*D1[L]
#                 V2111=V2111+T0000(ca,cb,cc,cd,AtomB,AtomA,AtomA,AtomA)*D2[I]*D1[J]*D1[K]*D1[L]
#                 V2121=V2121+T0000(ca,cb,cc,cd,AtomB,AtomA,AtomB,AtomA)*D2[I]*D1[J]*D2[K]*D1[L]
#                 V2211=V2211+T0000(ca,cb,cc,cd,AtomB,AtomB,AtomA,AtomA)*D2[I]*D2[J]*D1[K]*D1[L]
#                 V2221=V2221+T0000(ca,cb,cc,cd,AtomB,AtomB,AtomB,AtomA)*D2[I]*D2[J]*D2[K]*D1[L]
#                 V2222=V2222+T0000(ca,cb,cc,cd,AtomB,AtomB,AtomB,AtomB)*D2[I]*D2[J]*D2[K]*D2[L]
# print(sympy.N(V1111),sympy.N(V2111),sympy.N(V2121),sympy.N(V2211),sympy.N(V2221),sympy.N(V2222))

# BASIS "ao basis" SPHERICAL PRINT
# #BASIS SET: (3s) -> [1s]
# H    S
#       0.3425250914E+01       0.1543289673E+00
#       0.6239137298E+00       0.5353281423E+00
#       0.1688554040E+00       0.4446345422E+00
# END

# In[ ]:


CCF=np.array([[0.444635,0.535328,0.154329],
[0.109818,0.405771,2.22766]])
CCF.transpose()
import pandas as pd
pd.options.display.precision = 4
df = pd.DataFrame(CCF.transpose())
d2f=df.rename(columns={0: 'CA(i)',  1: 'DA(i)'},index={0: 1,  1: 2, 2:3}, inplace=True)
print(df.to_latex())


# In[ ]:


COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
zeta2=1.24
ZETAS=[1.24,1.24,1.24]
CA=[0,0,0]
DA=[0,0,0]
import numpy
PI=numpy.pi
[x*zeta2**2 for x in COEF[2]]
N=3
for ID in range(1):
    for i in range(N):
        #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
        CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
        DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
        print(CA[i],DA[i])


# In[ ]:


import numpy
import numpy as np
R_length=0.8649/0.529177
#R_length=0.96691406/0.529177
R=sympy.symbols("R",positive=True)
R_length=R
#R_length=1.46
atomA=[0,0,0]
atomB=[R_length,0,0]
atomC=[R_length*1/2,0,R_length*sympy.sqrt(3)/2]

ZETA1=2.0925
ZETA2=1.24
ZETA1=ZETA2
ZETA3=ZETA2
#
#
#
ZA=2.0
ZB=1.0
ZA=ZB
ZC=ZB
atoms=[atomA,atomB,atomC]
ZETAS=[ZETA1,ZETA2,ZETA3]
ZS=[ZA,ZB,ZC]
COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
DA=[0]*3
CA=[0]*3
DB=[0]*3
CB=[0]*3
DC=[0]*3
CC=[0]*3
DD=[0]*3
CD=[0]*3
PI=numpy.pi
TT=[[[[0 for _ in range(3)] for _  in range(3)] for _ in range(3)] for _ in range(3)]
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
            for LD in range(3):
                RA=[AX,AY,AZ]=atoms[ID]
                RB=[BX,BY,BZ]=atoms[JD]
                RC=[CX,CY,CZ]=atoms[KD]
                RD=[DX,DY,DZ]=atoms[LD]
                N=3
                for i in range(N):
                    #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
                    CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
                    DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
                    CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
                    DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)
                    CC[i]=EXPON[N-1][i]*(ZETAS[KD]**2)
                    DC[i]=COEF[N-1][i]*((2.0*CC[i]/PI)**0.75)
                    CD[i]=EXPON[N-1][i]*(ZETAS[LD]**2)
                    DD[i]=COEF[N-1][i]*((2.0*CD[i]/PI)**0.75)
                    
                N=3
                V=0
                for I in range(N):            
                    for J in range(N):
                        for K in range(N):
                            for L in range(N):
                                ca=CA[I]
                                cb=CB[J]
                                cc=CC[K]
                                cd=CD[L]
                                #print(ca,cb,cc,cd,sympy.N(T0000(ca,cb,cc,cd,RA,RB,RC,RD)))
                                
                                V=V+T0000(ca,cb,cc,cd,RA,RB,RC,RD)*DA[I]*DB[J]*DC[K]*DD[L]
                V=sympy.N(V)
                #print(RA,RB,RC,RD,V)
                TT[ID][JD][KD][LD]=V





# In[ ]:


def indexijkl(i,j,k,l):
    A=[(i,j,k,l),(j,i,k,l),(i,j,l,k),(j,i,l,k)]
    A+=[(k,l,i,j),(l,k,i,j),(k,l,j,i),(l,k,j,i)]
    A.sort()
    return A[0]


# In[ ]:


ALLTT=[]
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
            for LD in range(3):
                ALLTT.append(indexijkl(ID,JD,KD,LD))


# In[ ]:


from sympy.combinatorics import Permutation, PermutationGroup
F = Permutation(1,2)
R = Permutation(0,1,2)
D=Permutation()
G = PermutationGroup(F, R, D)
G.order()


# In[ ]:


GR=[]
for a in G.elements:
    GR.append(a)


# In[ ]:


S3=[ [(0,1),(1,0)],[(0,2),(2,1),(1,0)],[(0,1),(1,2),(2,0)], [],[(1,2),(2,1)],[(0,2),(2,0)]]


# In[ ]:


def replace(t,x):
    #print(t)
    s=list(t)
    #print(s)
    q=s
    for j in range(len(q)):
        for n,m in x:
            #print(q[j],":",n,m,x)
            if q[j]==n:
                q[j]=m
                #print("replace",q)
                break
            
 
    return tuple(q)


def getmin(t,S3):
    w=[replace(t,x) for x in S3]
    w=[indexijkl(i,j,k,l) for i,j,k,l, in w]
    #print(w)
    w.sort()
    i,j,k,l=w[0]
    return indexijkl(i,j,k,l)

getmin((0,1,1,1),S3)


# In[ ]:


W=[]
Z=[]
R=sympy.symbols("R",positive=True)
for i,j,k,l in set(ALLTT):
    print(i,j,k,l)
    expr=TT[i][j][k][l]
    #print(type(expr))
    #var=list(expr.free_symbols)[0]
    print((i,j,k,l),getmin((i,j,k,l),S3))
    #print(TT[i][j][k][l].subs([(R,1.5)]))
    W.append(getmin((i,j,k,l),S3))


# In[ ]:


set(Z)


# In[ ]:


TTTT=dict()
TTTTS=dict()
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
            for LD in range(3):
                t=(ID,JD,KD,LD)
                i,j,k,l=getmin(t,S3)
                print(t,"TT"+str(i)+str(j)+str(k)+str(l))
                key="TT"+str(i)+str(j)+str(k)+str(l)
                TTTT[t]=sympy.symbols(key)
                TTTTS[t]=key
                
                


# In[ ]:


str(TTTT.get((2,2,2,2)))


# In[ ]:


import itertools
from operator import itemgetter
W=[]
for a in itertools.product([0,1,2], repeat=4):
    i,j,k,l=a
    W.append([a,TT[i][j][k][l].subs(R,1.7),int((TTTTS.get(a).replace('T',''))),getmin((i,j,k,l),S3)])
    
W.sort(key=itemgetter(3))


# In[ ]:


len(W)


# In[ ]:


W


# In[ ]:


set(TTTT.values())


# In[ ]:


def replace(t,x):
    #print(t)
    s=list(t)
    #print(s)
    q=s
    for j in range(len(q)):
        for n,m in x:
            #print(q[j],":",n,m,x)
            if q[j]==n:
                q[j]=m
                #print("replace",q)
                break
            
 
    return tuple(q)


def getmin(t,S3):
    w=[replace(t,x) for x in S3]
    w=[indexijkl(i,j,k,l) for i,j,k,l, in w]
    print(w)
    w.sort()
    i,j,k,l=w[0]
    return indexijkl(i,j,k,l)

print(getmin((0,0,0,1),S3))
print(getmin((0,1,1,1),S3))
print(getmin(getmin((1,2,2,2),S3),S3))


# In[ ]:


TTTT


# In[ ]:


"""
            RAP=A2[J]*R/(A1[I]+A2[J])
            RAP2=RAP**2
            RBP2=(R-RAP)**2
            S12+=getS(A1[I],A2[J],R2)*D1[I]*D2[J]
            T11=T11+getT(A1[I],A1[J],0.0)*D1[I]*D1[J]
            #print(I,J,getT(A1[I],A1[J],0.0),D1[I],D1[J],T11)
            T12=T12+getT(A1[I],A2[J],R2)*D1[I]*D2[J]
            T22=T22+getT(A2[I],A2[J],0.0)*D2[I]*D2[J]
            V11A=V11A+V(A1[I],A1[J],0.0,0.0,ZA)*D1[I]*D1[J]
            V12A=V12A+V(A1[I],A2[J],R2,RAP2,ZA)*D1[I]*D2[J]
            V22A=V22A+V(A2[I],A2[J],0.0,R2,ZA)*D2[I]*D2[J]
            V11B=V11B+V(A1[I],A1[J],0.0,R2,ZB)*D1[I]*D1[J]
            V12B=V12B+V(A1[I],A2[J],R2,RBP2,ZB)*D1[I]*D2[J]
            V22B=V22B+V(A2[I],A2[J],0.0,0.0,ZB)*D2[I]*D2[J]
"""
def S000000(A,B,RA,RB):
#
#   OVERLAP INTEGRAL between exp(-A*|r-RA|^2) and exp(-B*|r-RB|^2)
#
    RAB2=sum([(c1-c2)**2 for c1,c2 in zip(RA,RB)])
    PI=np.pi
    #print(A,B,RA,RB,RAB2,(PI/(A+B))**1.5)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))
def GetRP(a,b,RA,RB):
    AX,AY,AZ=RA
    BX,BY,BZ=RB
    PX=(a*AX+b*BX)/(a+b)
    PY=(a*AY+b*BY)/(a+b)
    PZ=(a*AZ+b*BZ)/(a+b)
    return [PX,PY,PZ]

VAB_C=[[[0 for _ in range(3)] for _  in range(3)] for _ in range(3)]
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
                RA=[AX,AY,AZ]=atoms[ID]
                RB=[BX,BY,BZ]=atoms[JD]
                RC=[CX,CY,CZ]=atoms[KD]
                ZC=ZS[KD]
                N=3
                for i in range(N):
                    #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
                    CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
                    DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
                    CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
                    DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)
                    CC[i]=EXPON[N-1][i]*(ZETAS[KD]**2)
                    DC[i]=COEF[N-1][i]*((2.0*CC[i]/PI)**0.75)
                    CD[i]=EXPON[N-1][i]*(ZETAS[LD]**2)
                    DD[i]=COEF[N-1][i]*((2.0*CD[i]/PI)**0.75)
                    
                N=3
                V=0
                for I in range(N):            
                    for J in range(N):
                        
                                ca=CA[I]
                                cb=CB[J]
                                #V000000(a,b,RA,RB,RC)
                                V=V+V000000(ca,cb,RA,RB,RC)*DA[I]*DB[J]*(-ZC)
                V=sympy.N(V)
                #print(RA,RB,RC,RD,V)
                VAB_C[ID][JD][KD]=V

SAB=[[0 for _ in range(3)] for _  in range(3)]              
for ID in range(3):
    for JD in range(3):
        RA=[AX,AY,AZ]=atoms[ID]
        RB=[BX,BY,BZ]=atoms[JD]
        for i in range(N):
            #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
            CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
            DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
            CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
            DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)

        N=3
        V=0
        for I in range(N):            
            for J in range(N):
                        ca=CA[I]
                        cb=CB[J]
                        #V000000(a,b,RA,RB,RC)
                        V=V+S000000(ca,cb,RA,RB)*DA[I]*DB[J]
        V=sympy.N(V)
        #print(RA,RB,V)
        SAB[ID][JD]=V
        
KAB=[[0 for _ in range(3)] for _  in range(3)]              
for ID in range(3):
    for JD in range(3):
        RA=[AX,AY,AZ]=atoms[ID]
        RB=[BX,BY,BZ]=atoms[JD]
        for i in range(N):
            #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
            CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
            DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
            CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
            DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)

        N=3
        V=0
        for I in range(N):            
            for J in range(N):
                        ca=CA[I]
                        cb=CB[J]
                        #V000000(a,b,RA,RB,RC)
                        V=V+K000000(ca,cb,RA,RB)*DA[I]*DB[J]
        V=sympy.N(V)
        #print(RA,RB,V)
        KAB[ID][JD]=V


# In[ ]:


def FORMG():
#
# Calculates G matrix from density matrix and two-electron integrals
#
    for I in range(3):
        for J in range(3):
            G[I][J]=0
            for K in range(3):
                for L in range(3):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    G[I][J]+=P[K][L]*(TT[I][J][K][L]-0.5*TT[I][L][J][K])
    #print("G",G)
    return 



def SCF_SIMBOL3(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
# PREPARES THE ANALYTIC FORMULA OF THE TOTAL ENERGY.
#


    P=[[0 for _ in range(3)] for _ in range(3)]
    P2=[[0 for _ in range(3)] for _ in range(3)]
    G=[[0 for _ in range(3)] for _ in range(3)]
    G2=[[0 for _ in range(3)] for _ in range(3)]
    F=[[0 for _ in range(3)] for _ in range(3)]
    F2=[[0 for _ in range(3)] for _ in range(3)]
    H=[[0 for _ in range(3)] for _ in range(3)]
    x,y,z,u,v,w=symbols("x y z u v w")

    PI=np.pi
    CRIT=1.0e-4
    MAXIT=25
    ITER=0
    for I in range(3):
        for J in range(3):
            P[I][J]=0.
            

    P[0][0]=x*x*2
    P[0][1]=x*y*2
    P[0][2]=x*z*2
    P[1][0]=y*x*2
    P[1][1]=y*y*2
    P[1][2]=y*z*2
    P[2][0]=z*x*2
    P[2][1]=z*y*2
    P[2][2]=z*z*2

    for I in range(3):
        for J in range(3):
            G[I][J]=0
            G2[I][J]=0
            for K in range(3):
                for L in range(3):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    #print(I,J,K,L)
                    G[I][J]+=P[K][L]*TT[I][J][K][L]-0.5*P[K][L]*TT[I][L][J][K]
    H=[[0 for _ in range(3)] for _ in range(3)]
    for I in range(3):
        for J in range(3):
            H[I][J]=KAB[I][J]
            for K in range(3):
                H[I][J]+=VAB_C[I][J][K]

    for i in range(3):
        for j in range(3):
            F[i][j]=H[i][j]+G[i][j]

    EN=0
    for i in range(3):
        for j in range(3):
            EN+=0.5*P[i][j]*(H[i][j]+F[i][j])
    ENT=EN
    for i in range(3):
        for j in range(i+1,3):
            RPQ=[(c1-c2)**2 for c1,c2 in zip(atoms[i],atoms[j])]
            RPQ2=sum(RPQ)
            #print(RPQ2)
            ENT+=ZS[i]*ZS[j]/sympy.sqrt(RPQ2)
            


    return EN,ENT,F,F2,H,P
x,y,z,u,v,w=symbols("x y z u v w")
EN,ENT,FM,FM2,HM,PM=SCF_SIMBOL3(IOP,N,R,ZETA1,ZETA2,ZA,ZB)


# In[ ]:


def SCF_SIMBOL4(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
# PREPARES THE ANALYTIC FORMULA OF THE TOTAL ENERGY.
#


    P=[[0 for _ in range(3)] for _ in range(3)]
    P2=[[0 for _ in range(3)] for _ in range(3)]
    G=[[0 for _ in range(3)] for _ in range(3)]
    G2=[[0 for _ in range(3)] for _ in range(3)]
    F=[[0 for _ in range(3)] for _ in range(3)]
    F2=[[0 for _ in range(3)] for _ in range(3)]
    H=[[0 for _ in range(3)] for _ in range(3)]
    x,y,z,u,v,w=symbols("x y z u v w")

    PI=np.pi
    CRIT=1.0e-4
    MAXIT=25
    ITER=0
    for I in range(3):
        for J in range(3):
            P[I][J]=0.
    P[0][0]=x*x*2
    P[0][1]=x*y*2
    P[0][2]=x*z*2
    P[1][0]=y*x*2
    P[1][1]=y*y*2
    P[1][2]=y*z*2
    P[2][0]=z*x*2
    P[2][1]=z*y*2
    P[2][2]=z*z*2
    onehalf=sympy.sympify('0.5',rational=True)
    for I in range(3):
        for J in range(3):
            G[I][J]=0
            G2[I][J]=0
            for K in range(3):
                for L in range(3):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    #print(I,J,K,L)
                    #G[I][J]+=P[K][L]*TT[I][J][K][L]-0.5*P[K][L]*TT[I][L][J][K]
                    G[I][J]+=P[K][L]*TTTT[(I,J,K,L)]-onehalf*P[K][L]*TTTT[(I,L,J,K)]
    H=[[0 for _ in range(3)] for _ in range(3)]
    for I in range(3):
        for J in range(3):
            H[I][J]=KAB[I][J]
            for K in range(3):
                H[I][J]+=VAB_C[I][J][K]
    HO=symbols("H")
    HD=symbols("HD")
    for I in range(3):
        for J in range(3):
            H[I][J]=HO
            if I==J:
                H[I][J]=HD
    for i in range(3):
        for j in range(3):
            F[i][j]=H[i][j]+G[i][j]

    EN=0
    for i in range(3):
        for j in range(3):
            EN+=onehalf*P[i][j]*(H[i][j]+F[i][j])
    ENT=EN
    ZS=[1,1,1]
    for i in range(3):
        for j in range(i+1,3):
            RPQ=[(c1-c2)**2 for c1,c2 in zip(atoms[i],atoms[j])]
            RPQ2=sum(RPQ)
            #print(RPQ2)
            ENT+=ZS[i]*ZS[j]/sympy.sqrt(RPQ2)
            


    return EN,ENT,F,F2,H,P
x,y,z,u,v,w=symbols("x y z u v w")
TEN,TENT,TFM,TFM2,THM,TPM=SCF_SIMBOL4(IOP,N,R,ZETA1,ZETA2,ZA,ZB)


# In[ ]:


set(TTTT.values())


# In[ ]:


SAB


# In[ ]:


E


# In[ ]:


SS=[[0 for _ in range(3)] for _ in range(3)]
SO=symbols("S")
SD=symbols("SD")
for I in range(3):
    for J in range(3):
        SS[I][J]=SO
        if I==J:
            SS[I][J]=1

def GetVSW(vec,SAB,wec):
    V=0
    for i in range(len(vec)):
        for j in range(len(vec)):
            V+=vec[i]*SAB[i][j]*wec[j]
    return V            
            
def GetNormS(vec,SAB):
    V=0
    for i in range(len(vec)):
        for j in range(len(vec)):
            V+=vec[i]*SAB[i][j]*vec[j]
    return V

e,f=symbols("e f")
SAB[0][0]=1
SAB[1][1]=1
SAB[2][2]=1
OBJ=ENT-2*e*(GetNormS([x,y,z],SAB)-1)


# In[ ]:


OBJ=OBJ.subs(y,-2*x).subs(z,x)


# In[ ]:


vecs=[[x,x,x],[x,x,-2*x],[x,-x,0]]

for a in vecs:
    for b in vecs:
        print(a,b,GetVSW(a,SS,b))


# In[ ]:


TOBJ=TENT-2*e*(GetNormS([x,y,z],SS)-1)
TEV=GetNormS([x,y,z],TFM)
TNS=GetNormS([x,y,z],SS)


# In[ ]:


set(TTTT.values())


# In[ ]:


for a in vecs:
    p,q,r=a
    print([sympy.latex(expand(TEV.subs([(y,q),(z,r)]))),sympy.latex(TNS.subs([(y,q),(z,r)]))])


# In[ ]:


sympy.sympify(TOBJ.expand(),rational=True)


# HD=sympy.Symbol("HD")
# F0=_oh[302].subs(HD,0)-3/R
# F1=_oh[30].subs(y,x).subs(z,x).subs(HD,0)-3/R
# F2=_oh[30].subs(y,0).subs(z,-x).subs(HD,0)-3/R
# F3=_oh[30].subs(y,-2*x).subs(z,x).subs(HD,0)-3/R

# S0=sympy.poly(F0)
# S1=sympy.poly(F1)
# S2=sympy.poly(F2)
# S3=sympy.poly(F3)
# 

# #getF
# Fargs=str(S0.args[1:])
# #Fargs='(x, y, z,e)'
# stringQ='option(noredefine);LIB "solve.lib";option(redSB);\n'
# stringQ+='ring r=0,'+Fargs+',dp;\n'+'poly OBJ1='+str(F0)+';\n'
# #stringQ+='poly OBJ2='+str(F2)+';\n'
# #stringQ+='poly OBJ3='+str(F3)+';\n'
# stringQ+='list diffs;\n'
# stringQ+='for(int i=1;i<=nvars(r); i=i+1){diffs=insert(diffs,diff(OBJ1,var(i)));}\n'
# print(stringQ)

# In[ ]:


FM


# In[ ]:


OBJE=OBJ.expand()
OBJ=OBJE.subs(R,0.9/0.529177)
#OBJ=OBJE.subs(R,1.0/0.529177)
FMV=[[0,0,0],[0,0,0],[0,0,0]]
SABV=[[0,0,0],[0,0,0],[0,0,0]]
for i in range(3):
    for j in range(3):
        FMV[i][j]=FM[i][j].subs(R,0.9/0.529177)
        if (i!=j):
            SABV[i][j]=SAB[i][j].subs(R,0.9/0.529177)
        else:
            SABV[i][j]=1
FMV
SABV


# In[ ]:


def GetMdotV(M,S,V,e):
    R=[0]*len(V)
    for i in range(len(V)):
        for j in range(len(V)):
            R[i]+=M[i][j]*V[j]-e*S[i][j]*V[j]
    return R

#FMdotxy=GetMdotV(FM,SAB,[x,y,z],e)
#4*FMdotxy[0].expand()-OBJE.diff(x)
#4*FMdotxy[1].expand()-OBJE.diff(y)
#4*FMdotxy[2].expand()-OBJE.diff(z)


# In[ ]:


#[OBJE.diff(x).expand()-2*FMdotxy[0].expand(),
# OBJE.diff(y).expand()-2*FMdotxy[1].expand(),
# OBJE.diff(z).expand()-2*FMdotxy[2].expand()]


# In[ ]:


OBJ=OBJ.expand()
ENTS3=sympy.poly(sympy.N(OBJ))
OBJ


# In[ ]:


def getINT(x,N):
#
#  ROWND DOWN x*N AFTER THE DECIMAL POINT and get AN INTEGER M
#  THEN X is approximated by M/N. 
#
    return (int(np.floor(x*N)))

def getPowerProduct(args,tm):
    V=1
    for w,p in zip(list(args[1:]),tm):
        V*= w**p
    return V
OBJ=OBJ.expand()
ENTS3=sympy.poly(sympy.N(OBJ))
AT=ENTS3.terms()
getF=0
for tm in AT:
    #p0,p1,p2,p3,p4,p5,p6,p7=tm[0]
    cf=tm[1]
    #print(p0,p1,p2,cf)
    #getF+=x**p0* y**p1* z**p2* u**p3* v**p4* w**p5* e**p5* f**p7*getINT(cf,10000)
    getF+=getPowerProduct(ENTS3.args,tm[0])*getINT(cf,10000)


# In[ ]:


getF0=getF


# In[ ]:


getF=getF0.subs(y,0).subs(z,-x)


# In[ ]:


sympy.poly(getF).args


# In[ ]:


#getF="-20000*e*x**2 - 22288*e*x*y - 22288*e*x*z - 20000*e*y**2 - 22288*e*y*z - 20000*e*z**2 + 20000*e + 7746*x**4 + 14316*x**3*y + 14316*x**3*z + 18392*x**2*y**2 + 26758*x**2*y*z + 18392*x**2*z**2 - 31781*x**2 + 14316*x*y**3 + 26758*x*y**2*z + 26758*x*y*z**2 - 44637*x*y + 14316*x*z**3 - 44637*x*z + 7746*y**4 + 14316*y**3*z + 18392*y**2*z**2 - 31781*y**2 + 14316*y*z**3 - 44637*y*z + 7746*z**4 - 31781*z**2 + 17639"


# In[ ]:


#str(ENTS3.args[1:])


# In[ ]:


ENTS3


# In[ ]:


str(ENTS3.args[1:])


# In[ ]:


getF
Fargs=str(ENTS3.args[1:])
Fargs=str(sympy.poly(getF).args[1:])
#Fargs='(x, y, z,e)'
stringQ='option(noredefine);LIB "solve.lib";option(redSB);\n'
stringQ+='ring r=0,'+Fargs+',dp;\n'+'poly OBJ='+str(getF)+';\n'
stringQ+='list diffs;\n'
stringQ+='for(int i=1;i<=nvars(r); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}\n'
stringQ+='ideal I=0;\n'
stringQ+='for(int i=1;i<=nvars(r); i=i+1){I=I+diff(OBJ,var(i));}\n'
stringQ+='print(I);'
stringQ+='ideal SI=std(I);\n'
stringQ+='print(SI);'
stringQ+='ring s=0,'+Fargs+',lp;\n'
stringQ+='setring s;\n'
stringQ+='ideal j=fglm(r,SI);\n j;\n'
stringQ+='LIB "triang.lib";\n'
stringQ+='triangM(j);write(":w save_t.txt",triangM(j));\n' 
stringQ+='def R=triang_solve(j,50);\n'
stringQ+='setring R;rlist;\n'
stringQ+='poly OBJ=fetch(r,OBJ);\n\
ideal I=fetch(r,I);\n\
OBJ;\n\
list subste;\n\
for (i=1;i<=size(rlist);i=i+1)\
{\n\
list substv;\n\
\n\
poly OBJ2=OBJ;\n\
for (int k=1; k<=nvars(R); k=k+1)\n\
{\n\
 OBJ2=subst(OBJ2,var(k), rlist[i][k]);\n\
}\n\
substv=insert(substv,OBJ2);\n\
\n\
for (int l=1;l<=size(I);l=l+1)\n\
{\n\
 poly OBJ2=I[l];\n\
 for (int k=1; k<=nvars(R); k=k+1)\n\
 {\n\
  OBJ2=subst(OBJ2,var(k), rlist[i][k]);\n\
 }\n\
 substv=insert(substv,OBJ2,size(substv));\n\
}\n\
print("substv");\
print(substv);\n\
subste=insert(subste,substv,size(subste));\n\
}\n\
write(":w save_i.txt",rlist);\n\
write(":w save_e.txt",subste);\n\
print("subste");\n\
print(subste);\n\
quit;\n\
'

text_file = open("SCRIPT.txt", "w")
on = text_file.write(stringQ)
 
#close file
text_file.close()


# In[ ]:


import subprocess
cp = subprocess.run("Singular<SCRIPT.txt", shell=True,capture_output=True,text=True)
print("stdout:", cp.stdout)
print("stderr:", cp.stderr)


# In[ ]:


-0.61350847819359191236949919830515355101979163035887
-0.39883213214095405031135526651863929057839208322827
2965.8322467928081870400155371622972477842815164075
0.61350847819359191236949919830515355101979163035887
-0.39883213214095405031135526651863929057839208322827
2965.8322467928081870400155371622972477842815164075


# In[ ]:


tb=_ih[312].split("\n")
tb=np.array([float(x) for x in tb])
tb=[[tb[0],tb[1],tb[2]/10000],[tb[0],tb[1],tb[2]/10000]]
import pandas as pd;
df=pd.DataFrame(tb)
print(df.to_latex())


# In[ ]:


import copy
FMV2=copy.deepcopy(FMV)
xv=-0.39705054600483080889176715350196612593964157002994
for i in range(3):
    for j in range(3):
        FMV2[i][j]=FMV[i][j].subs(x,xv).subs(y,xv).subs(z,xv)

u,v,w,s,t=sympy.symbols("u v w s t")
FMV2        
getE2=GetNormS([u,v,w],FMV2)-s*(GetNormS([u,v,w],SABV)-1)-t*GetVSW([xv,xv,xv],SABV,[u,v,w])


def getINT(x,N):
#
#  ROWND DOWN x*N AFTER THE DECIMAL POINT and get AN INTEGER M
#  THEN X is approximated by M/N. 
#
    return (int(np.floor(x*N)))

def getPowerProduct(args,tm):
    V=1
    for w,p in zip(list(args[1:]),tm):
        V*= w**p
    return V
ENTS3=sympy.poly(getE2.expand())
AT=ENTS3.terms()


# In[ ]:


ENTS3


# In[ ]:


import copy
FMV2=copy.deepcopy(FMV)
xv=-0.39705054600483080889176715350196612593964157002994
for i in range(3):
    for j in range(3):
        FMV2[i][j]=FMV[i][j].subs(y,x).subs(z,x)

u,v,w,s,t, q=sympy.symbols("u v w s t q")
FMV2        
getE2=GetNormS([u,v,w],FMV2)-s*(GetNormS([u,v,w],SABV)-1)-t*GetVSW([x,x,x],SABV,[u,v,w])+q*(GetNormS([x,x,x],SABV)-1)


def getINT(x,N):
#
#  ROWND DOWN x*N AFTER THE DECIMAL POINT and get AN INTEGER M
#  THEN X is approximated by M/N. 
#
    return (int(np.floor(x*N)))

def getPowerProduct(args,tm):
    V=1
    for w,p in zip(list(args[1:]),tm):
        V*= w**p
    return V
ENTS3=sympy.poly(getE2.expand())
AT=ENTS3.terms()


# In[ ]:


FMV2


# In[ ]:


ENTS3.args


# In[ ]:


getF=0
for tm in AT:
    #p0,p1,p2,p3,p4,p5,p6,p7=tm[0]
    cf=tm[1]
    #print(p0,p1,p2,cf)
    #getF+=x**p0* y**p1* z**p2* u**p3* v**p4* w**p5* e**p5* f**p7*getINT(cf,10000)
    getF+=getPowerProduct(ENTS3.args,tm[0])*getINT(cf,10000)

type(sympy.sympify(getF))


# In[ ]:


sympy.latex(sympy.sympify(str(getF)))


# It would be too naive to substitute a digit to the ground state wavefunction $(x,x,x)$. We could use a more complicated objective function. Recall that the ground-state wavefunction is determined by 
# $
# (x,x,x)S(x,x,x)^T=1.
# $
# Then we construct the objective function for the virtual orbitals $(u,v,w)$ with constraints as follows: 
# $$
# (u,v,w)F(u,v,w)^T - s\cdot\left((u,v,w)S(u,v,v)^T-1\right)-t\cdot\left((x,x,x) S(u,v,w)^T\right)+q\cdot\left((x,x,x)S(x,x,x)^T-1\right)
# $$
# It determines both of the occupied and virtual orbitals in the ground state. The polynomial approximation is given by
# 
# $$63431 q x^{2} - 10000 q - 10000 s u^{2} - 11144 s u v - 11144 s u w - 10000 s v^{2} - 11144 s v w - 10000 s w^{2} + 10000 s - 21144 t u x - 21144 t v x - 21144 t w x + 46573 u^{2} x^{2} - 15891 u^{2} + 34956 u v x^{2} - 22319 u v + 34956 u w x^{2} - 22319 u w + 46573 v^{2} x^{2} - 15891 v^{2} + 34956 v w x^{2} - 22319 v w + 46573 w^{2} x^{2} - 15891 w^{2}$$
# Its optimum is also computed from an ideal (of dimension one) that is  composed of the partial derivatives of the objective function.  The Gr\"obner basis for this ideal is computed as follows:
# $
# \{u+v+w,
# t,
# 20805368s+679539,
# 70218117q+72737500,
# 1107v^2+1107vw+1107w^2-1250,
# 63431x^2-10000\}.
# $
# 
# 

# In[ ]:


getF
Fargs=str(ENTS3.args[1:])
#Fargs='(x, y, z,e)'
stringQ='option(noredefine);LIB "solve.lib";option(redSB);\n'
stringQ+='ring r=0,'+Fargs+',dp;\n'+'poly OBJ='+str(getF)+';\n'
stringQ+='list diffs;\n'
stringQ+='for(int i=1;i<=nvars(r); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}\n'
stringQ+='ideal I=0;\n'
stringQ+='for(int i=1;i<=nvars(r); i=i+1){I=I+diff(OBJ,var(i));}\n'
stringQ+='print(I);print("---");'
stringQ+='ideal SI=std(I);\n'
stringQ+='dim(SI);print(SI);'
stringQ+='ring s=0,'+Fargs+',lp;\n'
stringQ+='setring s;\n'
stringQ+='ideal j=fglm(r,SI);\n j;\n'
stringQ+='LIB "triang.lib";\n'
stringQ+='triangM(j);write(":w save_t.txt",triangM(j));\n' 
stringQ+='def R=triang_solve(j,50);\n'
stringQ+='setring R;rlist;\n'
stringQ+='poly OBJ=fetch(r,OBJ);\n\
ideal I=fetch(r,I);\n\
OBJ;\n\
list subste;\n\
for (i=1;i<=size(rlist);i=i+1)\
{\n\
list substv;\n\
\n\
poly OBJ2=OBJ;\n\
for (int k=1; k<=nvars(R); k=k+1)\n\
{\n\
 OBJ2=subst(OBJ2,var(k), rlist[i][k]);\n\
}\n\
substv=insert(substv,OBJ2);\n\
\n\
for (int l=1;l<=size(I);l=l+1)\n\
{\n\
 poly OBJ2=I[l];\n\
 for (int k=1; k<=nvars(R); k=k+1)\n\
 {\n\
  OBJ2=subst(OBJ2,var(k), rlist[i][k]);\n\
 }\n\
 substv=insert(substv,OBJ2,size(substv));\n\
}\n\
print("substv");\
print(substv);\n\
subste=insert(subste,substv,size(subste));\n\
}\n\
write(":w save_i.txt",rlist);\n\
write(":w save_e.txt",subste);\n\
print("subste");\n\
print(subste);\n\
quit;\n\
'
text_file = open("BSCRIPT.txt", "w")
on = text_file.write(stringQ)
 
#close file
text_file.close()

import subprocess
cp = subprocess.run(" Singular<BSCRIPT.txt", shell=True,capture_output=True,text=True)
print("stdout:", cp.stdout)
print("stderr:", cp.stderr)


# In[ ]:


text_file = open("SCRIPT.out.txt", "w")
on = text_file.write(cp.stdout)
 
#close file
text_file.close()


# In[ ]:


import csv
rowstd_dp=list()
with open('save_std_dp.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowstd_dp.append(t)
import csv
rowstd=list()
with open('save_std.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowstd.append(t)

from sympy import sympify, symbols,latex
x,y,z,e=symbols("x y z e")
string = rowt[0][1]
#print(latex(sympify(string)))
def rowstoexpr(rowt):
    wa=list()
    for  t in rowt:
        w=list()
        for s in t:
            #print(s)
            w.append(sympify(s))
        wa.append(w)
    return wa

exprs=rowstoexpr(rowstd)    


# In[ ]:


exprs[0][3].args


# In[ ]:


import pandas as pd
stdvars=pd.DataFrame()

stdvars["variables"]=[t.free_symbols for t in exprs[0]]
stdvars["length of expression"]=[len(str(t)) for t in exprs[0]]
stdvars["number of terms"]=[len(t.args) for t in exprs[0]]
#stdvars.to_latex()
stdvars


# In[ ]:


import csv
rowt=list()
with open('save_t.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowt.append(t[0:4])
        
import csv
rowTQ1=list()
with open('save_TQ1.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowTQ1.append(t[0:4])
import csv
rowTQ2=list()
with open('save_TQ2.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowTQ2.append(t[0:4])
print(rowt)
print(rowTQ1)
print(rowTQ2)


# In[ ]:


rowt[0][1]
from sympy import sympify, symbols,latex
x,y,z,e=symbols("x y z e")
string = rowt[0][1]
#print(latex(sympify(string)))

def rowstolatex(rowt):
    wa=list()
    for  t in rowt:
        w=list()
        for s in t:
            w.append("$"+latex(sympify(s))+"$")
        wa.append(w)
    import pandas as pd
    wapd=pd.DataFrame(wa)
    return wapd

rowstolatex(rowt)[0][1]


# In[ ]:





# In[ ]:


import csv
rowe=list()
with open('save_e.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        print(t)
        rowe.append(t[0:4])


# In[ ]:


import csv
row=list()
with open('save_i.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        print(t)
        row.append(t[0:4])


# In[ ]:


rows=[]
i=0
while 4*i+4<len(row):
    rows.append(row[4*i:4*i+4])
    i+=1


# In[ ]:


[len(t) for t in row]


# In[ ]:


rows2=[]
for x,y,z,e in row:
    try:
        p,q,r,s=[float(x),float(y),float(z),float(e)]
        rows2.append(['{:.5g}'.format(p),'{:.5g}'.format(q),'{:.5g}'.format(r),'{:.5g}'.format(s)])
    except:
        pass
rowse2=[]
for x,y,z,e in rowe:
    try:
        p,q,r,s=[float(x),float(y),float(z),float(e)]
        rowse2.append(['{:.5g}'.format(p),'{:.5g}'.format(q),'{:.5g}'.format(r),'{:.5g}'.format(s)])
    except:
        pass


# In[ ]:


rowse2


# In[ ]:


import pandas as pd
pd.options.display.precision = 4
df = pd.DataFrame(rows2)
dfe= pd.DataFrame(rowse2)


# In[ ]:


df[4]=[float(x)/10000 for x in dfe[0]]


# In[ ]:





# In[ ]:


print(df.to_latex())


# In[ ]:


df[0][0]



==> advancedcomputations.tex <==
#!/usr/bin/env python
# coding: utf-8

# These Python programs compute the electronic structure of H3+ in the equilateral triangle. 
# 
# The atoms are indexed by A, B, and C, or a, b, and c.
# The STO-3G are determined by the parameters ZETA, COEFF, and EXPON. 
# 
# (1) SZ-SIM-H3P-RHF
#       For RHF computation.  
#       The variables (x,y,z) : the LCAO coefficients of 1s orbitals on the vertices.
#       The variable e : the orbital energy
#       The variable R: the length of the edges, fixed at a positive number.
# 
# (2) SZ-SIM-H3P-UHF
#       For UHF computation.  
#       The variables (x,y,z) : the LCAO coefficients of 1s orbitals on the vertices, for spin alpha
#       The variables e : the orbital energy, for spin alpha
#       The variables (u,v,w) : the LCAO coefficients of 1s orbitals on the vertices, for spin beta
#       The variables f : the orbital energy, for spin beta
#       The variable R: the length of the edges, fixed at a positive number.
# 
# (3) SZ-SIM-H3P-RHF-DeterminR, SZ-SIM-H3P-RHF-DeterminR-Version2
#       The variables (x,x,x) : the LCAO coefficients of 1s orbitals on the vertices.
#       The variable e : the orbital energy
#       The variable R: the length of the edges, to be optimized as well as other variables.

# In[1]:


#!/usr/bin/env python
# coding: utf-8

#
#  SUNDRY DEFINITIONS OF WORKING VARIABLES.
#
import networkx as nx

IG=nx.DiGraph() 
from sympy import symbols, Function,expand,sqrt
import numpy as np
import copy
from itertools import combinations_with_replacement, permutations,product

S12,T11,T12,T22,V11A,V12A,V22A,V11B,V12B,V22B,V1111,V2111,V2121,V2211,V2221,V2222=[0 for _ in range(16)]

S=[[0 for _ in range(2)] for _ in range(2)]
X=[[0 for _ in range(2)] for _  in range(2)]
NM=[[0 for _ in range(2)] for _  in range(2)]
XT=[[0 for _ in range(2)] for _ in  range(2)]
H=[[0 for _ in range(2)] for _ in  range(2)]
F=[[0 for _ in range(2)] for _ in  range(2)]
P=[[0 for _ in range(2)] for _  in range(2)]
G=[[0 for _ in range(2)] for _ in  range(2)]
F2=[[0 for _ in range(2)] for _ in  range(2)]
P2=[[0 for _ in range(2)] for _  in range(2)]
G2=[[0 for _ in range(2)] for _ in  range(2)]

C=[[0 for _ in range(2)] for _ in  range(2)]
FPRIME=[[0 for _ in range(2)] for _  in range(2)]
CPRIME=[[0 for _ in range(2)] for _  in range(2)]
P=[[0 for _ in range(2)] for _  in range(2)]
ODLPP=[[0 for _ in range(2)] for _  in range(2)]
E=[[0 for _ in range(2)] for _  in range(2)]
TT=[[[[0 for _ in range(2)] for _  in range(2)] for _ in range(2)] for _ in range(2)]

IOP=2
N=3
ZETA1=2.0925
ZETA2=1.24
ZA=2.0
ZB=1.0
#
#  Atomic distance R
#
R=symbols("R",positive=True)
#
#  Wavefunction (x,y) for alpha spin
#  Wavefunction (v,w) for beta spin
#
v, w = symbols("v w")
x, y = symbols("x y")


#
# In the following, we compute the atomic orbital integrals by the Gaussian orbital 
#  exp(-A*|r-RA|^2),exp(-A*|B-RB|^2),exp(-C*|r-RC|^2),exp(-D*|r-RD|^2)
#

import sympy as sympy
from sympy import symbols, Function,expand,core,sqrt
import numpy as np


def F0(ARG):
#
# BOYS F0 FUNCTIOM
#
    PI = sympy.pi
    if  type(ARG)==float and ARG < 1.0e-6:
        return 1 -ARG/3.
    if  type(ARG)==sympy.core.numbers.Zero and ARG < 1.0e-6:
        return 1 -ARG/3.
    else:
        #print("F0:ARG",ARG)
        if ARG!=sympy.S.Zero:
            return sympy.sqrt(PI/ARG)*sympy.erf(sqrt(ARG))/2
        else:
            return 1
    
def S000000(A,B,RA,RB):
#
#   OVERLAP INTEGRAL between exp(-A*|r-RA|^2) and exp(-B*|r-RB|^2)
#
    RAB2=sum([(c1-c2)**2 for c1,c2 in zip(RA,RB)])
    PI=np.pi
    print(A,B,RAB2,(PI/(A+B))**1.5)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def getS(A,B,RAB2):
#
# Calculates the overlap matrix between exp(-A*|r-RA|^2) and exp(-A*|B-RB|^2)
# WHEN RAB2=|RA-RB|^2
#
    PI=np.pi
    print(A,B,RAB2,(PI/(A+B))**1.5)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def K000000(A,B,RA,RB):
    RAB2=sum([(c1-c2)**2 for c1,c2 in zip(RA,RB)])
    PI=np.pi
    return A*B/(A+B)*(3.0-2.0*A*B*RAB2/(A+B))*(PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))   

def getT(A,B,RAB2):
#
# Calculates the kinetic energy
#  between exp(-A*|r-RA|^2) and exp(-B*|r-RB|^2)
# WHEN RAB2=|RA-RB|^2
#
    PI=np.pi
    return A*B/(A+B)*(3.0-2.0*A*B*RAB2/(A+B))*(PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def V(A,B,RAB2,RCP2,ZC):
#
#  CALCULATES UN-NORMALIZED NUCLEAR ATTRACTION INTEGRALS
#
    PI=np.pi
    V=2.0*PI/(A+B)*F0((A+B)*RCP2)*sympy.exp(-A*B*RAB2/(A+B))
    return -V*ZC

def TWOE(A,B,C,D,RAB2,RCD2,RPQ2):
#
# CALCULATES TWO-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
# A,B,C,D ARE THE EXPONENTS ALPHA, BETA, ETC.
# RAB2 EQUALS SQUARED DISTANCE BETWEEN CENTER A AND CENTER B, ETC.
#
# The integrand is the product of those functions.
#   exp(-A*|r1-RA|^2),exp(-B*|r1-RB|^2),1/|r1-r2|, exp(-C*|r2-RC|^2),exp(-D*|r2-RD|^2)
# when RB=RA and RD=RC.
#
#
    PI=np.pi
    return 2.0*(PI**2.5)/((A+B)*(C+D)*np.sqrt(A+B+C+D))*F0((A+B)*(C+D)*RPQ2/(A+B+C+D))*sympy.exp(-A*B*RAB2/(A+B)-C*D*RCD2/(C+D))

    
def BOYS(N,X):
#
#  BOYS FUNCTION F_N(X)
#
    if N==0:
        return F0(X)
    else:
        Z=Symbol("Z")
        f=F0(Z)
        for _ in range(N):
            f=f.diff(Z)*(-1)
        return f.subs(Z,X)
    
def KXYZAB(a,b,RA,RB):
    mu=a*b/(a+b)
    RAB=[(c1-c2)**2 for c1,c2 in zip(RA,RB)]
    RAB2=sum(RAB)
    return sympy.exp(-mu*RAB2)

def T0000(a,b,c,d,RA,RB,RC,RD):
#
# CALCULATES TWO-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
# a,b,c,d ARE THE EXPONENTS ALPHA, BETA, ETC.
# RAB2 EQUALS SQUARED DISTANCE BETWEEN CENTER A AND CENTER B, ETC.
#
# The integrand is the product of those functions.
#   exp(-a*|r1-RA|^2),exp(-b*|r1-RB|^2),1/|r1-r2|, exp(-c*|r2-RC|^2),exp(-d*|r2-RD|^2)
#
#
    def MF0(ARG):
    #
    # BOYS F0 FUNCTIOM
    #
        PI = sympy.pi
        if  type(ARG)==float and ARG < 1.0e-6:
            return 1 -ARG/3.
        if  type(ARG)==sympy.core.numbers.Zero and ARG < 1.0e-6:
            return 1 -ARG/3.
        else:
            #print("F0:ARG",ARG)
            if ARG!=sympy.S.Zero:
                return sympy.sqrt(PI/ARG)*sympy.erf(sqrt(ARG))/2
            else:
                return 1
    p=a+b
    q=c+d
    RP=[(a*c1+b*c2)/(a+b) for c1,c2 in zip(RA,RB)]
    RQ=[(c*c1+d*c2)/(c+d) for c1,c2 in zip(RC,RD)]
    alpha=p*q/(p+q)
    PI=sympy.pi
    RPQ=[(c1-c2)**2 for c1,c2 in zip(RP,RQ)]
    RPQ2=sum(RPQ)
    return 2*PI**(2.5)/p/q/sympy.sqrt(p+q)*KXYZAB(a,b,RA,RB)*KXYZAB(c,d,RC,RD)*MF0(alpha*RPQ2)

def V000000(a,b,RA,RB,RC):
#
# CALCULATES ONE-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
#
#  The integrand is the product of those functions.
#   exp(-a*|r-RA|^2),exp(-b*|r-RB|^2),1/|r-RC|
#  
    p=a+b
    PI=sympy.pi
    RP=[(a*c1+b*c2)/(a+b) for c1,c2 in zip(RA,RB)]
    RPC=[(c1-c2)**2 for c1,c2 in zip(RP,RC)]
    RPC2=sum(RPC)
    return 2*PI/p*KXYZAB(a,b,RA,RB)*BOYS(0,p*RPC2)

def TN0000(N,a,b,c,d,RA,RB,RC,RD):
#
#  This function is the simplest case of the so-Called auxilary function THETA(N;000 000 000 000)
#  in Obara-Saika Schme for two-electron integrals.
#
    if N<0:
        return 0
    p=a+b
    q=c+d
    RP=[(a*c1+b*c2)/(a+b) for c1,c2 in zip(RA,RB)]
    RQ=[(c*c1+d*c2)/(c+d) for c1,c2 in zip(RC,RD)]
    alpha=p*q/(p+q)
    PI=sympy.pi
    RPQ=[(c1-c2)**2 for c1,c2 in zip(RP,RQ)]
    RPQ2=sum(RPQ)
    return 2*PI**(2.5)/p/q/sympy.sqrt(p+q)*KXYZAB(a,b,RA,RB)*KXYZAB(c,d,RC,RD)*BOYS(N,alpha*RPQ2)


#
#  TEST
#
AX,AY,AZ,BX,BY,BZ,CX,CY,CZ,DX,DY,DZ=symbols("AX AY AZ BX BY BZ CX CY CZ DX DY DZ")
z1,z2,z3,z4=symbols("z1 z2 z3 z4")
f=T0000(z1,z2,z3,z4,[AX,AY,AZ],[BX,BY,BZ],[CX,CY,CZ],[DX,DY,DZ])
print(f)


#
# TEST
#
((S000000(z1,z2,[AX,AY,AZ],[BX,BY,BZ]).diff(AX)).diff(AX)).subs([(BX,AX),(BY,AY),(BZ,AZ)])


# #
# # PERFORMANCE TEST CONCERNING DIFFERENTIATION (TO GENERATE TWO-ELECTRON INTERGRALS OF P-ORBITALS)
# #
# #
# import time,random
# ALL=[]
# for va in [AX,AY,AZ]:
#     for vb in [BX,BY,BZ]:
#         for vc in [CX,CY,CZ]:
#             for vd in [DX,DY,DZ]:
#                 z1,z2,z3,z4=symbols("z1 z2 z3 z4")
#                 z1,z2,z3,z4=[random.random() for _ in range(4)]
#                 #z1,z2,z3,z4=[z1,z2,random.random(),random.random()]
#                 f0=T0000(z1,z2,z3,z4,[AX,AY,AZ],[BX,BY,BZ],[CX,CY,CZ],[DX,DY,DZ])
#                 #print(f)
#                 #print(va,vb,vc,vd)
#                 start=time.time()
# 
#                 f1=f0.diff(va)
#                 
#                 f2=f1.diff(vb)
#                 f3=f2.diff(vc)
#                 f4=f3.diff(vd)
#                 
#                 end=time.time()
# 
#                 print("time=",end-start)
#                 ALL.append([f0,f1,f2,f3,f4])




from sympy import Function, Symbol
TN=Function("TN0000")
UNDEF=Function("UNDEF")

from sympy import Number
class FMA(Function):
    """
    FMA(x, y, z) = x*y + z
    """
    @classmethod
    def eval(cls, x, y, z):
        # Number is the base class of Integer, Rational, and Float
        if all(isinstance(i, Number) for i in [x, y, z]):
           return x*y + z
    def doit(self, deep=True, **hints):
        x, y, z = self.args
        # Recursively call doit() on the args whenever deep=True.
        # Be sure to pass deep=True and **hints through here.
        if deep:
            x = x.doit(deep=deep, **hints)
            y = y.doit(deep=deep, **hints)
            z = z.doit(deep=deep, **hints)
        return x*y + z
    
    


# # Obara-Saika Scheme for Two-electron integrals



#
# We prepare dummy expressions for THE FUNCTIONS TN0000(N,a,b,c,d,RA,RB,RC,RD): TNS[0],TNS[1],...., WHICH SHALL BE USED LATER
#  THEY ARE AUXILLARY INTEGRALS, AND IF N=0 , THEY ARE THE TWO-ELECTRON INTGRALS.
#

TNSTRING=''
for i in range(11):
    TNSTRING+= 'TN'+str(i)+' '
TNS=symbols(TNSTRING)
def TN(N):
    return TNS[N]




#
#  INITIALIZATION OF OBARA-SAIKA
#
#INTEGRALALL=dict()
#for i in range(11):
#    INTEGRALALL[(i,0,0,0,0,0,0,0,0,0,0,0,0)]=TN(i)
    
IG=nx.DiGraph() 




#
#  EACH NUCLEI IS STATIONED IN THE 3D CARTESIAN SPACE:r=(x,y,z)
#  THE COORDINATES ARE REPRESENTED AS RA=(XA,YA,ZB)
#  THE DIFFERENCE ARE REPRESENTED BY XPA=XP-XA, YPQ=YP-YQ, ZAB=ZA-AB, AND SO ON.
#
#  WE START FROM SPHERICAL GAUSSIAN FUNCTIONS : (a,RA)=exp(-a|r-RA|^2),exp(-b|r-RB|^2),exp(-c|r-RC|^2),exp(-d|r-rB|^2).
#
#
#
XPA, XPQ, XCD, XAB=symbols("XPA XPQ XCD XAB")
YPA, YPQ,YCD, YAB=symbols("YPA YPQ YCD YAB")
ZPA, ZPQ, ZCD, ZAB=symbols("ZPA ZPQ ZCD ZAB")
XQC, YQC, ZQC=symbols("XQC YQC ZQC")
#
#
#  [(a,RA;r1),(b,Rb;r1)| 1/|r1-r2| | (c,Rd);r2,(d,RD;r2)] 
#
#
#  We put p=a*b/(a+b);q=c*d/(c+d); alpha=p*q/(p+q).
#  Provisionally p,q are left as they are without substitution.
#  At the end of the computation, we have to replace them.
#
a,b,c,d=symbols("a b c d")
p,q=symbols("p q")
alpha=symbols("alpha")

#
#  We compute the integrals using general Cartesian Gaussian functions:
#   (x-XA)^i (y-YA)^j (z-ZA)^j exp(-a|r-RA|^2)
#
#  VIZ.
#   [(i1,j1,k1,a,RA),(i2,j2,k2,b,RB)|1/|r1-r2||(i3,j3,k3,d,RC),(i4,j4,k4,d,RD)]
#
#  For brevity, we write:
#   i=(i1,i2,i3), j=(j1,j2,j3), k=(k1,k2,k3),
# 
#  To compute the auxillary integdals T(N,i,j,k,l) we lift from T(N,i=0.j=0,k=0,z=0)
#  WHEN N=0 THEY GIVE THE TWO-ELECTRON INTEGRALS; OBARA-SAIKA RECURSION USES THEM WITH N>=1.
#
#  BY VERTICAL RECUSION IN OBARA-SAIKA, WE COMPUTE 
#  (N: i+1 0 0 0 ) from (N: i 0 0 0) , (N+1 i 0 0 0) , (N i-1 0 0 0), (N+1 i 0 0 0)
#
#  WHERE i+1 is the every possible move from (i1,i2,i3) by adding one or zero to each of (i1,i2,i3), 
#  except zero-move. 
#
#  THE FOLLOWING FUNCTION LIFTS UP IN D=X/Y/Z DIRECTIONS AND COMPUTES THE INTGRALS.

def VERTICAL(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,INFO=0):
    alpha=p*q/(p+q)
    
    if D=="X":
        assert (j1==j2==j3==k1==k2==k3==l1==l2==l3==0),print(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,"X")
        #print("X")
        key0=(N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key1=(N+1,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key2=(N,i1-1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key3=(N+1,i1-1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        keyn=(N,i1+1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        i_d,k_d=i1,k1
        #print(keyn)
        DPA=XPA
        DPQ=XPQ
    if D=="Y":
        #print("Y")
        assert (j1==j2==j3==k1==k2==k3==l1==l2==l3==0),print(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,"X")
        key0=(N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key1=(N+1,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key2=(N,i1,i2-1,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key3=(N+1,i1,i2-1,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        keyn=(N,i1,i2+1,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        i_d,k_d=i2,k2
        #print(keyn)
        DPA=YPA
        DPQ=YPQ
    if D=="Z":
        assert (j1==j2==j3==k1==k2==k3==l1==l2==l3==0),print(D,N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3,"X")
        #print("Z")
        key0=(N,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key1=(N+1,i1,i2,i3,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key2=(N,i1,i2,i3-1,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        key3=(N+1,i1,i2,i3-1,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        keyn=(N,i1,i2,i3+1,j1,j2,j3,k1,k2,k3,l1,l2,l3)
        i_d,k_d=i3,k3
        #print(keyn)
        DPA=ZPA
        DPQ=ZPQ
    if None!=integrals_all.get(keyn):
        return
    
    data0=integrals_all.get(key0)
    data1=integrals_all.get(key1)
    data2=integrals_all.get(key2)
    data3=integrals_all.get(key3)
    #print(key0,key1,key2,key3)
    #print(data0,data1,data2,data3)
    nx.add_star(IG, [keyn,key0, key1, key2, key3])
    if min(list(key2))<0:
        data2=0
        integrals_all[key2]=0
    if min(list(key3))<0:
        data3=0
        integrals_all[key3]=0
    if data0==None:
        #print("data 0 requested")
        requested_keys[key0]=key0
    if data1==None:
        #print("data 1 requested")
        requested_keys[key1]=key1
    if data2==None:
        #print("data 2 requested")
        requested_keys[key2]=key2
    if data3==None:
        #print("data 3 requested")
        requested_keys[key3]=key3
    #print(requested_keys.keys())
    if data0!=None and data1!=None and data2!=None and data3!=None:
        if (INFO==1):
            print(keyn,"WRITTEN")
        integrals_all[keyn]= DPA*data0-alpha/p*DPQ*data1+i_d/2/p*(data2-alpha/p*data3)
    else:
        if (INFO==1):
            print(keyn,"NOT WRITTEN")
            print(key0,key1,key2,key3)
            print(data0,data1,data2,data3)
        else:
            pass
    return
    
#
#  The indices of the integrals which are required, but has not yet been computed.
#
requested_keys=dict()
        
#
#  The dictionary of computed integrals
#
integrals_all=dict()
for i in range(11):
    integrals_all[(i,0,0,0,0,0,0,0,0,0,0,0,0)]=TN(i)        


# V1111=0.0
# V2111=0.0
# V2121=0.0
# V2211=0.0
# V2221=0.0
# V2222=0.0
# N=3
# COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
# EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
# AtomA=[0,0,0]
# R_length=0.9/0.529177
# AtomB=[R_length,0,0]
# ZETA1=2.0925
# ZETA2=1.24
# ZETA1=ZETA2
# A1=[0]*N
# D1=[0]*N
# A2=[0]*N
# D2=[0]*N
# PI=np.pi
# for i in range(N):
#     #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
#     A1[i]=EXPON[N-1][i]*ZETA1**2
#     D1[i]=COEF[N-1][i]*((2.0*A1[i]/PI)**0.75)
#     A2[i]=EXPON[N-1][i]*(ZETA2**2)
#     D2[i]=COEF[N-1][i]*((2.0*A2[i]/PI)**0.75)
# for I in range(N):
#     for J in range(N):
#         for K in range(N):
#             for L in range(N):
#                 RAP=A2[I]*R/(A2[I]+A1[J])
#                 RBP=R-RAP
#                 RAQ=A2[K]*R/(A2[K]+A1[L])
#                 RBQ=R-RAQ
#                 RPQ=RAP-RAQ
#                 RAP2=RAP*RAP
#                 RBP2=RBP*RBP
#                 RAQ2=RAQ*RAQ
#                 RBQ2=RBQ*RBQ
#                 RPQ2=RPQ*RPQ
#                 """
#                 V1111=V1111+TWOE(A1[I],A1[J],A1[K],A1[L],0.0,0.0,0.0)*D1[I]*D1[J]*D1[K]*D1[L]
#                 V2111=V2111+TWOE(A2[I],A1[J],A1[K],A1[L],R2,0.0,RAP2)*D2[I]*D1[J]*D1[K]*D1[L]
#                 V2121=V2121+TWOE(A2[I],A1[J],A2[K],A1[L],R2,R2,RPQ2)*D2[I]*D1[J]*D2[K]*D1[L]
#                 V2211=V2211+TWOE(A2[I],A2[J],A1[K],A1[L],0.0,0.0,R2)*D2[I]*D2[J]*D1[K]*D1[L]
#                 V2221=V2221+TWOE(A2[I],A2[J],A2[K],A1[L],0.0,R2,RBQ2)*D2[I]*D2[J]*D2[K]*D1[L]
#                 V2222=V2222+TWOE(A2[I],A2[J],A2[K],A2[L],0.0,0.0,0.0)*D2[I]*D2[J]*D2[K]*D2[L]
#                 """
#                 ca=A1[I]
#                 cb=A1[J]
#                 cc=A1[K]
#                 cd=A1[L]
#                 """
#                 V1111=V1111+T0000(A1[I],A1[J],A1[K],A1[L],AtomA,AtomA,AtomA,AtomA)*D1[I]*D1[J]*D1[K]*D1[L]
#                 V2111=V2111+T0000(A2[I],A1[J],A1[K],A1[L],AtomB,AtomA,AtomA,AtomA)*D2[I]*D1[J]*D1[K]*D1[L]
#                 V2121=V2121+T0000(A2[I],A1[J],A2[K],A1[L],AtomB,AtomA,AtomB,AtomA)*D2[I]*D1[J]*D2[K]*D1[L]
#                 V2211=V2211+T0000(A2[I],A2[J],A1[K],A1[L],AtomB,AtomB,AtomA,AtomA)*D2[I]*D2[J]*D1[K]*D1[L]
#                 V2221=V2221+T0000(A2[I],A2[J],A2[K],A1[L],AtomB,AtomB,AtomB,AtomA)*D2[I]*D2[J]*D2[K]*D1[L]
#                 V2222=V2222+T0000(A2[I],A2[J],A2[K],A2[L],AtomB,AtomB,AtomB,AtomB)*D2[I]*D2[J]*D2[K]*D2[L]
#                 """
#                 V1111=V1111+T0000(ca,cb,cc,cd,AtomA,AtomA,AtomA,AtomA)*D1[I]*D1[J]*D1[K]*D1[L]
#                 V2111=V2111+T0000(ca,cb,cc,cd,AtomB,AtomA,AtomA,AtomA)*D2[I]*D1[J]*D1[K]*D1[L]
#                 V2121=V2121+T0000(ca,cb,cc,cd,AtomB,AtomA,AtomB,AtomA)*D2[I]*D1[J]*D2[K]*D1[L]
#                 V2211=V2211+T0000(ca,cb,cc,cd,AtomB,AtomB,AtomA,AtomA)*D2[I]*D2[J]*D1[K]*D1[L]
#                 V2221=V2221+T0000(ca,cb,cc,cd,AtomB,AtomB,AtomB,AtomA)*D2[I]*D2[J]*D2[K]*D1[L]
#                 V2222=V2222+T0000(ca,cb,cc,cd,AtomB,AtomB,AtomB,AtomB)*D2[I]*D2[J]*D2[K]*D2[L]
# print(sympy.N(V1111),sympy.N(V2111),sympy.N(V2121),sympy.N(V2211),sympy.N(V2221),sympy.N(V2222))

# BASIS "ao basis" SPHERICAL PRINT
# #BASIS SET: (3s) -> [1s]
# H    S
#       0.3425250914E+01       0.1543289673E+00
#       0.6239137298E+00       0.5353281423E+00
#       0.1688554040E+00       0.4446345422E+00
# END

# In[2]:


CCF=np.array([[0.444635,0.535328,0.154329],
[0.109818,0.405771,2.22766]])
CCF.transpose()
import pandas as pd
pd.options.display.precision = 4
df = pd.DataFrame(CCF.transpose())
d2f=df.rename(columns={0: 'CA(i)',  1: 'DA(i)'},index={0: 1,  1: 2, 2:3}, inplace=True)
print(df.to_latex())


# COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
# EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
# zeta2=1.24
# 
# [x*zeta2**2 for x in COEF[2]]
# N=3
# for ID in range(1):
#     for i in range(N):
#         #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
#         CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
#         DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
#         print(CA[i],DA[i])

# In[3]:


import numpy
import numpy as np
R_length=0.8649/0.529177
#R_length=0.96691406/0.529177
R=sympy.symbols("R",positive=True)
R_length=R
#R_length=1.46
atomA=[0,0,0]
atomB=[R_length,0,0]
atomC=[R_length*1/2,0,R_length*sympy.sqrt(3)/2]

ZETA1=2.0925
ZETA2=1.24
ZETA1=ZETA2
ZETA3=ZETA2
#
#
#
ZA=2.0
ZB=1.0
ZA=ZB
ZC=ZB
atoms=[atomA,atomB,atomC]
ZETAS=[ZETA1,ZETA2,ZETA3]
ZS=[ZA,ZB,ZC]
COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
DA=[0]*3
CA=[0]*3
DB=[0]*3
CB=[0]*3
DC=[0]*3
CC=[0]*3
DD=[0]*3
CD=[0]*3
PI=numpy.pi
TT=[[[[0 for _ in range(3)] for _  in range(3)] for _ in range(3)] for _ in range(3)]
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
            for LD in range(3):
                RA=[AX,AY,AZ]=atoms[ID]
                RB=[BX,BY,BZ]=atoms[JD]
                RC=[CX,CY,CZ]=atoms[KD]
                RD=[DX,DY,DZ]=atoms[LD]
                N=3
                for i in range(N):
                    #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
                    CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
                    DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
                    CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
                    DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)
                    CC[i]=EXPON[N-1][i]*(ZETAS[KD]**2)
                    DC[i]=COEF[N-1][i]*((2.0*CC[i]/PI)**0.75)
                    CD[i]=EXPON[N-1][i]*(ZETAS[LD]**2)
                    DD[i]=COEF[N-1][i]*((2.0*CD[i]/PI)**0.75)
                    
                N=3
                V=0
                for I in range(N):            
                    for J in range(N):
                        for K in range(N):
                            for L in range(N):
                                ca=CA[I]
                                cb=CB[J]
                                cc=CC[K]
                                cd=CD[L]
                                #print(ca,cb,cc,cd,sympy.N(T0000(ca,cb,cc,cd,RA,RB,RC,RD)))
                                
                                V=V+T0000(ca,cb,cc,cd,RA,RB,RC,RD)*DA[I]*DB[J]*DC[K]*DD[L]
                V=sympy.N(V)
                #print(RA,RB,RC,RD,V)
                TT[ID][JD][KD][LD]=V





# In[4]:


#
#  The index of two-electron integral [ij|kl]: get the minimal one in the equivalence.
#
def indexijkl(i,j,k,l):
    A=[(i,j,k,l),(j,i,k,l),(i,j,l,k),(j,i,l,k)]
    A+=[(k,l,i,j),(l,k,i,j),(k,l,j,i),(l,k,j,i)]
    A.sort()
    return A[0]


# In[5]:


ALLTT=[]
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
            for LD in range(3):
                ALLTT.append(indexijkl(ID,JD,KD,LD))


# In[6]:


from sympy.combinatorics import Permutation, PermutationGroup
F = Permutation(1,2)
R = Permutation(0,1,2)
D=Permutation()
G = PermutationGroup(F, R, D)
G.order()


# In[7]:


GR=[]
for a in G.elements:
    GR.append(a)


# In[8]:


#
# Define operations according to the triangular symmetry. (S3)
#
S3=[ [(0,1),(1,0)],[(0,2),(2,1),(1,0)],[(0,1),(1,2),(2,0)], [],[(1,2),(2,1)],[(0,2),(2,0)]]


# In[9]:


#
#  Replace the entries in a tuple t accorging to a permutation x.
#
def replace(t,x):
    #print(t)
    s=list(t)
    #print(s)
    q=s
    for j in range(len(q)):
        for n,m in x:
            #print(q[j],":",n,m,x)
            if q[j]==n:
                q[j]=m
                #print("replace",q)
                break
            
 
    return tuple(q)

#
#  Conduct the permutations (according to a set S3) to a tuple t; Wfind the minimal element among the generated elements.
#
def getmin(t,S3):
    w=[replace(t,x) for x in S3]
    w=[indexijkl(i,j,k,l) for i,j,k,l, in w]
    #print(w)
    w.sort()
    i,j,k,l=w[0]
    return indexijkl(i,j,k,l)

getmin((0,1,1,1),S3)


# In[10]:


W=[]
Z=[]
R=sympy.symbols("R",positive=True)
for i,j,k,l in set(ALLTT):
    print(i,j,k,l)
    expr=TT[i][j][k][l]
    #print(type(expr))
    #var=list(expr.free_symbols)[0]
    print((i,j,k,l),getmin((i,j,k,l),S3))
    #print(TT[i][j][k][l].subs([(R,1.5)]))
    W.append(getmin((i,j,k,l),S3))


# In[11]:


set(Z)


# In[12]:


#
# Checks. For a [ij|kl], get the minimal representative.
#
TTTT=dict()
TTTTS=dict()
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
            for LD in range(3):
                t=(ID,JD,KD,LD)
                i,j,k,l=getmin(t,S3)
                print(t,"TT"+str(i)+str(j)+str(k)+str(l))
                key="TT"+str(i)+str(j)+str(k)+str(l)
                TTTT[t]=sympy.symbols(key)
                TTTTS[t]=key
                
                


# In[13]:


str(TTTT.get((2,2,2,2)))


# In[14]:


import itertools
from operator import itemgetter
W=[]
for a in itertools.product([0,1,2], repeat=4):
    i,j,k,l=a
    W.append([a,TT[i][j][k][l].subs(R,1.5),int((TTTTS.get(a).replace('T',''))),getmin((i,j,k,l),S3)])
    
W.sort(key=itemgetter(3))


# In[15]:


W


# In[16]:


#
# We get six representatives. 
#
set(TTTT.values())


# In[ ]:


def replace(t,x):
    #print(t)
    s=list(t)
    #print(s)
    q=s
    for j in range(len(q)):
        for n,m in x:
            #print(q[j],":",n,m,x)
            if q[j]==n:
                q[j]=m
                #print("replace",q)
                break
            
 
    return tuple(q)


def getmin(t,S3):
    w=[replace(t,x) for x in S3]
    w=[indexijkl(i,j,k,l) for i,j,k,l, in w]
    print(w)
    w.sort()
    i,j,k,l=w[0]
    return indexijkl(i,j,k,l)

print(getmin((0,0,0,1),S3))
print(getmin((0,1,1,1),S3))
print(getmin(getmin((1,2,2,2),S3),S3))


# In[18]:


"""
            RAP=A2[J]*R/(A1[I]+A2[J])
            RAP2=RAP**2
            RBP2=(R-RAP)**2
            S12+=getS(A1[I],A2[J],R2)*D1[I]*D2[J]
            T11=T11+getT(A1[I],A1[J],0.0)*D1[I]*D1[J]
            #print(I,J,getT(A1[I],A1[J],0.0),D1[I],D1[J],T11)
            T12=T12+getT(A1[I],A2[J],R2)*D1[I]*D2[J]
            T22=T22+getT(A2[I],A2[J],0.0)*D2[I]*D2[J]
            V11A=V11A+V(A1[I],A1[J],0.0,0.0,ZA)*D1[I]*D1[J]
            V12A=V12A+V(A1[I],A2[J],R2,RAP2,ZA)*D1[I]*D2[J]
            V22A=V22A+V(A2[I],A2[J],0.0,R2,ZA)*D2[I]*D2[J]
            V11B=V11B+V(A1[I],A1[J],0.0,R2,ZB)*D1[I]*D1[J]
            V12B=V12B+V(A1[I],A2[J],R2,RBP2,ZB)*D1[I]*D2[J]
            V22B=V22B+V(A2[I],A2[J],0.0,0.0,ZB)*D2[I]*D2[J]
"""
def S000000(A,B,RA,RB):
#
#   OVERLAP INTEGRAL between exp(-A*|r-RA|^2) and exp(-B*|r-RB|^2)
#
    RAB2=sum([(c1-c2)**2 for c1,c2 in zip(RA,RB)])
    PI=np.pi
    #print(A,B,RA,RB,RAB2,(PI/(A+B))**1.5)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))
def GetRP(a,b,RA,RB):
    AX,AY,AZ=RA
    BX,BY,BZ=RB
    PX=(a*AX+b*BX)/(a+b)
    PY=(a*AY+b*BY)/(a+b)
    PZ=(a*AZ+b*BZ)/(a+b)
    return [PX,PY,PZ]

VAB_C=[[[0 for _ in range(3)] for _  in range(3)] for _ in range(3)]
for ID in range(3):
    for JD in range(3):
        for KD in range(3):
                RA=[AX,AY,AZ]=atoms[ID]
                RB=[BX,BY,BZ]=atoms[JD]
                RC=[CX,CY,CZ]=atoms[KD]
                ZC=ZS[KD]
                N=3
                for i in range(N):
                    #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
                    CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
                    DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
                    CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
                    DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)
                    CC[i]=EXPON[N-1][i]*(ZETAS[KD]**2)
                    DC[i]=COEF[N-1][i]*((2.0*CC[i]/PI)**0.75)
                    CD[i]=EXPON[N-1][i]*(ZETAS[LD]**2)
                    DD[i]=COEF[N-1][i]*((2.0*CD[i]/PI)**0.75)
                    
                N=3
                V=0
                for I in range(N):            
                    for J in range(N):
                        
                                ca=CA[I]
                                cb=CB[J]
                                #V000000(a,b,RA,RB,RC)
                                V=V+V000000(ca,cb,RA,RB,RC)*DA[I]*DB[J]*(-ZC)
                V=sympy.N(V)
                #print(RA,RB,RC,RD,V)
                VAB_C[ID][JD][KD]=V

SAB=[[0 for _ in range(3)] for _  in range(3)]              
for ID in range(3):
    for JD in range(3):
        RA=[AX,AY,AZ]=atoms[ID]
        RB=[BX,BY,BZ]=atoms[JD]
        for i in range(N):
            #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
            CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
            DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
            CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
            DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)

        N=3
        V=0
        for I in range(N):            
            for J in range(N):
                        ca=CA[I]
                        cb=CB[J]
                        #V000000(a,b,RA,RB,RC)
                        V=V+S000000(ca,cb,RA,RB)*DA[I]*DB[J]
        V=sympy.N(V)
        #print(RA,RB,V)
        SAB[ID][JD]=V
        
KAB=[[0 for _ in range(3)] for _  in range(3)]              
for ID in range(3):
    for JD in range(3):
        RA=[AX,AY,AZ]=atoms[ID]
        RB=[BX,BY,BZ]=atoms[JD]
        for i in range(N):
            #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
            CA[i]=EXPON[N-1][i]*ZETAS[ID]**2
            DA[i]=COEF[N-1][i]*((2.0*CA[i]/PI)**0.75)
            CB[i]=EXPON[N-1][i]*(ZETAS[JD]**2)
            DB[i]=COEF[N-1][i]*((2.0*CB[i]/PI)**0.75)

        N=3
        V=0
        for I in range(N):            
            for J in range(N):
                        ca=CA[I]
                        cb=CB[J]
                        #V000000(a,b,RA,RB,RC)
                        V=V+K000000(ca,cb,RA,RB)*DA[I]*DB[J]
        V=sympy.N(V)
        #print(RA,RB,V)
        KAB[ID][JD]=V


# In[19]:


def FORMG():
#
# Calculates G matrix from density matrix and two-electron integrals
#
    for I in range(3):
        for J in range(3):
            G[I][J]=0
            for K in range(3):
                for L in range(3):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    G[I][J]+=P[K][L]*(TT[I][J][K][L]-0.5*TT[I][L][J][K])
    #print("G",G)
    return 



def SCF_SIMBOL3(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
# PREPARES THE ANALYTIC FORMULA OF THE TOTAL ENERGY.
#


    P=[[0 for _ in range(3)] for _ in range(3)]
    P2=[[0 for _ in range(3)] for _ in range(3)]
    G=[[0 for _ in range(3)] for _ in range(3)]
    G2=[[0 for _ in range(3)] for _ in range(3)]
    F=[[0 for _ in range(3)] for _ in range(3)]
    F2=[[0 for _ in range(3)] for _ in range(3)]
    H=[[0 for _ in range(3)] for _ in range(3)]
    x,y,z,u,v,w=symbols("x y z u v w")

    PI=np.pi
    CRIT=1.0e-4
    MAXIT=25
    ITER=0
    for I in range(3):
        for J in range(3):
            P[I][J]=0.
    P[0][0]=x*x*2
    P[0][1]=x*y*2
    P[0][2]=x*z*2
    P[1][0]=y*x*2
    P[1][1]=y*y*2
    P[1][2]=y*z*2
    P[2][0]=z*x*2
    P[2][1]=z*y*2
    P[2][2]=z*z*2

    for I in range(3):
        for J in range(3):
            G[I][J]=0
            G2[I][J]=0
            for K in range(3):
                for L in range(3):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    #print(I,J,K,L)
                    G[I][J]+=P[K][L]*TT[I][J][K][L]-0.5*P[K][L]*TT[I][L][J][K]
    H=[[0 for _ in range(3)] for _ in range(3)]
    for I in range(3):
        for J in range(3):
            H[I][J]=KAB[I][J]
            for K in range(3):
                H[I][J]+=VAB_C[I][J][K]

    for i in range(3):
        for j in range(3):
            F[i][j]=H[i][j]+G[i][j]

    EN=0
    for i in range(3):
        for j in range(3):
            EN+=0.5*P[i][j]*(H[i][j]+F[i][j])
    ENT=EN
    for i in range(3):
        for j in range(i+1,3):
            RPQ=[(c1-c2)**2 for c1,c2 in zip(atoms[i],atoms[j])]
            RPQ2=sum(RPQ)
            #print(RPQ2)
            ENT+=ZS[i]*ZS[j]/sympy.sqrt(RPQ2)
            


    return EN,ENT,F,F2,H,P
x,y,z,u,v,w=symbols("x y z u v w")
EN,ENT,FM,FM2,HM,PM=SCF_SIMBOL3(IOP,N,R,ZETA1,ZETA2,ZA,ZB)


# In[20]:


def SCF_SIMBOL4(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
# PREPARES THE ANALYTIC FORMULA OF THE TOTAL ENERGY.
#


    P=[[0 for _ in range(3)] for _ in range(3)]
    P2=[[0 for _ in range(3)] for _ in range(3)]
    G=[[0 for _ in range(3)] for _ in range(3)]
    G2=[[0 for _ in range(3)] for _ in range(3)]
    F=[[0 for _ in range(3)] for _ in range(3)]
    F2=[[0 for _ in range(3)] for _ in range(3)]
    H=[[0 for _ in range(3)] for _ in range(3)]
    x,y,z,u,v,w=symbols("x y z u v w")

    PI=np.pi
    CRIT=1.0e-4
    MAXIT=25
    ITER=0
    for I in range(3):
        for J in range(3):
            P[I][J]=0.
    P[0][0]=x*x*2
    P[0][1]=x*y*2
    P[0][2]=x*z*2
    P[1][0]=y*x*2
    P[1][1]=y*y*2
    P[1][2]=y*z*2
    P[2][0]=z*x*2
    P[2][1]=z*y*2
    P[2][2]=z*z*2
    onehalf=sympy.sympify('0.5',rational=True)
    for I in range(3):
        for J in range(3):
            G[I][J]=0
            G2[I][J]=0
            for K in range(3):
                for L in range(3):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    #print(I,J,K,L)
                    #G[I][J]+=P[K][L]*TT[I][J][K][L]-0.5*P[K][L]*TT[I][L][J][K]
                    G[I][J]+=P[K][L]*TTTT[(I,J,K,L)]-onehalf*P[K][L]*TTTT[(I,L,J,K)]
    H=[[0 for _ in range(3)] for _ in range(3)]
    for I in range(3):
        for J in range(3):
            H[I][J]=KAB[I][J]
            for K in range(3):
                H[I][J]+=VAB_C[I][J][K]
    HO=symbols("H")
    HD=symbols("HD")
    for I in range(3):
        for J in range(3):
            H[I][J]=HO
            if I==J:
                H[I][J]=HD
    for i in range(3):
        for j in range(3):
            F[i][j]=H[i][j]+G[i][j]

    EN=0
    for i in range(3):
        for j in range(3):
            EN+=onehalf*P[i][j]*(H[i][j]+F[i][j])
    ENT=EN
    ZS=[1,1,1]
    for i in range(3):
        for j in range(i+1,3):
            RPQ=[(c1-c2)**2 for c1,c2 in zip(atoms[i],atoms[j])]
            RPQ2=sum(RPQ)
            #print(RPQ2)
            ENT+=ZS[i]*ZS[j]/sympy.sqrt(RPQ2)
            


    return EN,ENT,F,F2,H,P
x,y,z,u,v,w=symbols("x y z u v w")
TEN,TENT,TFM,TFM2,THM,TPM=SCF_SIMBOL4(IOP,N,R,ZETA1,ZETA2,ZA,ZB)


# In[21]:


set(TTTT.values())


# In[22]:


SAB


# In[23]:


E


# In[24]:


SS=[[0 for _ in range(3)] for _ in range(3)]
HO=symbols("S")
HD=symbols("SD")
for I in range(3):
    for J in range(3):
        SS[I][J]=HO
        if I==J:
            SS[I][J]=1

def GetVSW(vec,SAB,wec):
    V=0
    for i in range(len(vec)):
        for j in range(len(vec)):
            V+=vec[i]*SAB[i][j]*wec[j]
    return V            
            
def GetNormS(vec,SAB):
    V=0
    for i in range(len(vec)):
        for j in range(len(vec)):
            V+=vec[i]*SAB[i][j]*vec[j]
    return V

e,f=symbols("e f")
SAB[0][0]=1
SAB[1][1]=1
SAB[2][2]=1
OBJ=ENT-2*e*(GetNormS([x,y,z],SAB)-1)


# In[25]:


vecs=[[x,x,x],[x,x,-2*x],[x,-x,0]]

for a in vecs:
    for b in vecs:
        print(a,b,GetVSW(a,SS,b))


# In[26]:


TOBJ=TENT-2*e*(GetNormS([x,y,z],SS)-1)
TEV=GetNormS([x,y,z],TFM)
TNS=GetNormS([x,y,z],SS)


# In[27]:


set(TTTT.values())


# In[28]:


for a in vecs:
    p,q,r=a
    print([sympy.latex(expand(TEV.subs([(y,q),(z,r)]))),sympy.latex(TNS.subs([(y,q),(z,r)]))])


# In[29]:


sympy.sympify(TOBJ.expand(),rational=True)


# In[30]:


OBJE=OBJ.expand()
OBJ=OBJE.subs(R,0.9/0.529177)
#OBJ=OBJE.subs(R,1.0/0.529177)


# In[31]:


def GetMdotV(M,S,V,e):
    R=[0]*len(V)
    for i in range(len(V)):
        for j in range(len(V)):
            R[i]+=M[i][j]*V[j]-e*S[i][j]*V[j]
    return R

#FMdotxy=GetMdotV(FM,SAB,[x,y,z],e)
#4*FMdotxy[0].expand()-OBJE.diff(x)
#4*FMdotxy[1].expand()-OBJE.diff(y)
#4*FMdotxy[2].expand()-OBJE.diff(z)


# In[32]:


#[OBJE.diff(x).expand()-2*FMdotxy[0].expand(),
# OBJE.diff(y).expand()-2*FMdotxy[1].expand(),
# OBJE.diff(z).expand()-2*FMdotxy[2].expand()]


# In[33]:


def getINT(x,N):
#
#  ROWND DOWN x*N AFTER THE DECIMAL POINT and get AN INTEGER M
#  THEN X is approximated by M/N. 
#
    return (int(np.floor(x*N)))

def getPowerProduct(args,tm):
    V=1
    for w,p in zip(list(args[1:]),tm):
        V*= w**p
    return V
OBJ=OBJ.expand()
ENTS3=sympy.poly(sympy.N(OBJ))
AT=ENTS3.terms()
getF=0
for tm in AT:
    #p0,p1,p2,p3,p4,p5,p6,p7=tm[0]
    cf=tm[1]
    #print(p0,p1,p2,cf)
    #getF+=x**p0* y**p1* z**p2* u**p3* v**p4* w**p5* e**p5* f**p7*getINT(cf,10000)
    getF+=getPowerProduct(ENTS3.args,tm[0])*getINT(cf,10000)


# In[34]:


getF="-20000*e*x**2 - 22288*e*x*y - 22288*e*x*z - 20000*e*y**2 - 22288*e*y*z - 20000*e*z**2 + 20000*e + 7746*x**4 + 14316*x**3*y + 14316*x**3*z + 18392*x**2*y**2 + 26758*x**2*y*z + 18392*x**2*z**2 - 31781*x**2 + 14316*x*y**3 + 26758*x*y**2*z + 26758*x*y*z**2 - 44637*x*y + 14316*x*z**3 - 44637*x*z + 7746*y**4 + 14316*y**3*z + 18392*y**2*z**2 - 31781*y**2 + 14316*y*z**3 - 44637*y*z + 7746*z**4 - 31781*z**2 + 17639"


# In[35]:


#str(ENTS3.args[1:])


# In[36]:


#getF


# In[37]:


str(ENTS3.args[1:])


# In[38]:


getF
#Fargs=str(ENTS3.args[1:])
Fargs='(x, y, z,e)'
stringQ='option(noredefine);LIB "solve.lib";option(redSB);\n'
stringQ+='ring r=0,'+Fargs+',dp;\n'+'poly OBJ='+str(getF)+';\n'
stringQ+='list diffs;\n'
stringQ+='for(int i=1;i<=nvars(r); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}\n'
stringQ+='ideal I=0;\n'
stringQ+='for(int i=1;i<=nvars(r); i=i+1){I=I+diff(OBJ,var(i));}\n'
stringQ+='print(I);'
stringQ+='ideal SI=std(I);\n'
stringQ+='print(SI);'
stringQ+='ring s=0,'+Fargs+',lp;\n'
stringQ+='setring s;\n'
stringQ+='ideal j=fglm(r,SI);\n j;\n'
stringQ+='LIB "triang.lib";\n'
stringQ+='triangM(j);write(":w save_t.txt",triangM(j));\n' 
stringQ+='def R=triang_solve(j,50);\n'
stringQ+='setring R;rlist;\n'
stringQ+='poly OBJ=fetch(r,OBJ);\n\
ideal I=fetch(r,I);\n\
OBJ;\n\
list subste;\n\
for (i=1;i<=size(rlist);i=i+1)\
{\n\
list substv;\n\
\n\
poly OBJ2=OBJ;\n\
for (int k=1; k<=nvars(R); k=k+1)\n\
{\n\
 OBJ2=subst(OBJ2,var(k), rlist[i][k]);\n\
}\n\
substv=insert(substv,OBJ2);\n\
\n\
for (int l=1;l<=size(I);l=l+1)\n\
{\n\
 poly OBJ2=I[l];\n\
 for (int k=1; k<=nvars(R); k=k+1)\n\
 {\n\
  OBJ2=subst(OBJ2,var(k), rlist[i][k]);\n\
 }\n\
 substv=insert(substv,OBJ2,size(substv));\n\
}\n\
print("substv");\
print(substv);\n\
subste=insert(subste,substv,size(subste));\n\
}\n\
write(":w save_i.txt",rlist);\n\
write(":w save_e.txt",subste);\n\
print("subste");\n\
print(subste);\n\
quit;\n\
'

text_file = open("SCRIPT.txt", "w")
on = text_file.write(stringQ)
 
#close file
text_file.close()


# In[39]:


import subprocess
#cp = subprocess.run("Singular<SCRIPT-H3+.txt", shell=True,capture_output=True,text=True)
cp = subprocess.run("wsl Singular<SCRIPT.txt", shell=True,capture_output=True,text=True)
print("stdout:", cp.stdout)
print("stderr:", cp.stderr)


# In[40]:


text_file = open("SCRIPT.out.txt", "w")
on = text_file.write(cp.stdout)
 
#close file
text_file.close()


# In[41]:


import csv
rowstd_dp=list()
with open('save_std_dp.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowstd_dp.append(t)
import csv
rowstd=list()
with open('save_std.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowstd.append(t)

from sympy import sympify, symbols,latex
x,y,z,e=symbols("x y z e")
#string = rowt[0][1]
#print(latex(sympify(string)))
def rowstoexpr(rowt):
    wa=list()
    for  t in rowt:
        w=list()
        for s in t:
            #print(s)
            w.append(sympify(s))
        wa.append(w)
    return wa

exprs=rowstoexpr(rowstd)    


# In[42]:


import re
re.sub('[0-9]{2,}',"(C)",rowstd[0][1])
#rowstd[0][1].replace('[0-9]{2,}',"C")


# In[43]:


[re.sub('[0-9]{2,}',"()",str(t)) for t in exprs[0]]


# In[44]:


import pandas as pd
import numpy as np
stdvars=pd.DataFrame()

stdvars["variables"]=[t.free_symbols for t in exprs[0]]
#stdvars["length of expression"]=[len(str(t)) for t in exprs[0]]
#stdvars["number of terms"]=[len(t.args) for t in exprs[0]]
stdvars["formula"]=[re.sub('[0-9]{2,}',"()",str(t)) for t in exprs[0]]
stdvars.index = np.arange(1, len(stdvars)+1)
print(stdvars.to_latex())
#stdvars


# In[ ]:





# In[45]:


import csv
rowt=list()
with open('save_t.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowt.append(t[0:4])
        
import csv
rowTQ1=list()
with open('save_TQ1.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowTQ1.append(t[0:4])
import csv
rowTQ2=list()
with open('save_TQ2.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        #print(t)
        rowTQ2.append(t[0:4])
print(rowt)
print(rowTQ1)
print(rowTQ2)


# In[ ]:


rowt[0][1]
from sympy import sympify, symbols,latex
x,y,z,e=symbols("x y z e")
string = rowt[0][1]
#print(latex(sympify(string)))

def rowstolatex(rowt):
    wa=list()
    for  t in rowt:
        w=list()
        for s in t:
            w.append("$"+latex(sympify(s))+"$")
        wa.append(w)
    import pandas as pd
    wapd=pd.DataFrame(wa)
    return wapd

rowstolatex(rowt)[0][1]


# In[ ]:





# In[ ]:


import csv
rowe=list()
with open('save_e.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        print(t)
        rowe.append(t[0:4])


# In[ ]:


import csv
row=list()
with open('save_i.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        print(t)
        row.append(t[0:4])


# In[ ]:


rows=[]
i=0
while 4*i+4<len(row):
    rows.append(row[4*i:4*i+4])
    i+=1


# In[ ]:


[len(t) for t in row]


# In[ ]:


rows2=[]
for x,y,z,e in row:
    try:
        p,q,r,s=[float(x),float(y),float(z),float(e)]
        rows2.append(['{:.5g}'.format(p),'{:.5g}'.format(q),'{:.5g}'.format(r),'{:.5g}'.format(s)])
    except:
        pass
rowse2=[]
for x,y,z,e in rowe:
    try:
        p,q,r,s=[float(x),float(y),float(z),float(e)]
        rowse2.append(['{:.5g}'.format(p),'{:.5g}'.format(q),'{:.5g}'.format(r),'{:.5g}'.format(s)])
    except:
        pass


# In[ ]:


rowse2


# In[ ]:


import pandas as pd
pd.options.display.precision = 4
df = pd.DataFrame(rows2)
dfe= pd.DataFrame(rowse2)


# In[ ]:


df[4]=[float(x)/10000 for x in dfe[0]]


# In[ ]:





# In[ ]:


print(df.to_latex())


# In[ ]:


df[0][0]


# In[ ]:


import csv
rowqb=list()
with open('save_qbase.txt', 'r') as file:
    reader = csv.reader(file)
    for t in reader:
        print(t)
        rowqb.append(t)
len(rowqb[0])


# In[ ]:


26**2


# In[ ]:


# importing csv module
import csv
import numpy as np
rowm=list()
with open('matrix.csv','r') as file:
    reader = csv.reader(file)
    i=0
    for t in reader:
        #print(t)
        i+=1
        rowm.append(t)
#rowm
from fractions import Fraction
mx=[[0 for i in range(26)] for j in range(26)]
my=[[0 for i in range(26)] for j in range(26)]
mz=[[0 for i in range(26)] for j in range(26)]
me=[[0 for i in range(26)] for j in range(26)]
for mt, i,j,v in rowm:
    #print(i,j,v)
    v=float(Fraction(v))
    try:
        if mt=="mx":
            mx[int(i)-1][int(j)-1]=v
        if mt=="my":
            my[int(i)-1][int(j)-1]=v
        if mt=="mz":
            mz[int(i)-1][int(j)-1]=v
        if mt=="me":
            me[int(i)-1][int(j)-1]=v
    except:
        pass
    
mx=np.array(mx).transpose()
my=np.array(my).transpose()
mz=np.array(mz).transpose()
me=np.array(me).transpose()


# In[ ]:


es


# In[ ]:


me
import numpy as np
import numpy.linalg as LA


ee,ve=LA.eig(np.array(me))
ve=ve.transpose()
ex,vx=LA.eig(np.array(mx))
vx=vx.transpose()
ey,vy=LA.eig(np.array(my))
vy=vy.transpose()
ez,vz=LA.eig(np.array(mz))
vz=vz.transpose()

mxyze=np.dot(np.dot(np.dot(mx,my),mz),me)
ef,vf=LA.eig(np.array(mz))
vf=vf.transpose()

es=ee
vs=ve
lcs=list()

for i in range(len(es)):
    if np.abs(es[i].imag)<1.0e-10 and es[i].real>-1 and es[i].real >-0.36:
        print(es[i],[np.dot(np.dot(tt,vs[i]),np.conj(vs[i])) for tt in [mx,my,mz,me]])
        print(i,vs[i])
        lcs.append(i)
lcs   


# In[ ]:


mxyze=np.dot(np.dot(np.dot(mx,my),mz),me)
ef,vf=LA.eig(np.array(mxyze))
vf=vf.transpose()
for e,v in zip(ef,vf):
    print([np.dot(np.dot(tt,v),np.conj(v)) for tt in [mx,my,mz,me]])


# In[ ]:


[es[i] for i in [0, 3, 7, 14, 19, 24]]


# In[ ]:


from scipy.linalg import eigh
ic=0
jc=0
lcs=[16,21]
#lcs=[0, 3, 7, 14, 19,  24]
#lcs=[4, 8, 11, 15, 20, 25]

#lcs=[0, 3, 14]

s=np.array([[0.+0.j for _ in range(len(lcs))] for _ in range(len(lcs))])

h=np.array([[0.+0.j for _ in range(len(lcs))]for _ in range(len(lcs))])
for tt in [mx,my,mz]:
    ic=0
    for i in lcs:
        jc=0
        for j in lcs:
            h[ic][jc]=np.dot(np.dot(tt,vs[i]),np.conj(vs[j]))
            s[ic][jc]=np.dot(vs[i],np.conj(vs[j]))
            jc+=1
        ic+=1
    print("h",h)
    print("s",s)
    print("eighs",eigh(h,s))
    print("eigh",LA.eig(h))


# In[ ]:


h


# In[ ]:


[e for e in ee if np.abs(e.imag)<1.0e-10]


# In[ ]:


vs[25,:]


# In[ ]:


FL=list()
for v in vs:
    Found=False
    for x in v:
        if np.abs(x.imag)>1.0e-10:
            Found=True
            break
    FL.append(Found)

def IsComplexArray(v):
    Found=False
    for x in v:
        if np.abs(x.imag)>1.0e-10:
            Found=True
            break
    return Found
    


# In[ ]:


for p in [mx,my,mz,me]:
    for q in [mx,my,mz,me]:
        
        A=np.dot(np.array(p),np.array(q))-np.dot(np.array(q),np.array(p))
        print([np.max(A),np.min(A)])


# In[ ]:


es,vs=LA.eig(me)
vs=vs.transpose()
for i in range(len(es)):
    print(es[i],vs[i])


# In[ ]:


vs[:,25]


# In[ ]:


a=np.array(mz)
es,vs=LA.eig(np.array(a))
vs=vs.transpose()
print(es)
w=list()
for v in vs:
        print(IsComplexArray(v))
        print("v=",v)
        ev=np.dot(np.conj(v),np.dot((me),(v)))
        xv=np.dot(np.conj(v),np.dot((mx),(v)))
        yv=np.dot(np.conj(v),np.dot((my),(v)))
        zv=np.dot(np.conj(v),np.dot((mz),(v)))
        print([ev,xv,yv,zv])



# In[ ]:


IR=list()
for i in range(len(mx)):
    e=w[-1][i]
    if np.abs(e.imag)<1.0e-10:
        IR.append(i)
#        print([ww[i] for ww in w])
#            print(ww[i])
z=[]
for x in w:
    z.append([x[i] for i in IR])
z=np.array(z).transpose()
z


# In[ ]:


import csv
rowmx=list()
with open('save_mx.txt', 'r') as file:
    reader = csv.reader(file)
    i=0
    for t in reader:
        print()
        i+=1
        rowmx.append(t)
rowmx


# In[ ]:


rowm[1]


# In[ ]:


import csv

import pandas as pd
locallist=list()
for i in range(1,5):
    with open('trlist'+str(i)+'.txt', 'r') as file:
        rowqb=list()
        reader = csv.reader(file)
        for t in reader:
            print(t)
            rowqb.append(t)
    #print(len(rowqb[0]))
    x=rowqb[0]
    leng=int(len(x)/4)

    for j in range(leng):
        locallist.append([x[4*j],x[4*j+1],x[4*j+2],x[4*j+3],'T['+str(i)+']'])
        
locallist    


# In[ ]:


def Rewrite(x):
    r=list()
    for xx in x:
        try:
            a=float(xx)
            b="{0:.4f}".format(a)
            r.append(b)
        except:
            r.append(xx)
    return r

df=pd.DataFrame([Rewrite(local) for local in locallist])
     
with open("sample.txt", "w") as fileobj:
    fileobj.write(df.to_latex())



==> name.tex <==
#!/usr/bin/env python
# coding: utf-8

# In[ ]:


#materials projectのREST APIを用いるためのmodule
from pymatgen.ext.matproj import MPRester
#バンド構造のプロット用
get_ipython().run_line_magic('matplotlib', 'inline')
from pymatgen.electronic_structure.plotter import BSPlotter


# In[ ]:


#自分のAPIkeyを指定
a = MPRester("5xospsIpXSGq9sQ3")
#欲しい材料のidを指定して、http通信で取得。CuAlO2(mp-3784を取得します)
bs = a.get_bandstructure_by_material_id("mp-3748")


# In[ ]:


bss = a.get_data("Ti-Ba-O")


# In[ ]:


bss


# In[ ]:


bs.get_band_gap()
#plotter = BSPlotter(bs)
#plotter.get_plot().show()


# In[ ]:


import itertools
import pandas as pd

symbols=["Ti","Ba","O","Dy","Mg","Mn","Si","C",""]
# 希ガスを除く第２周期までの元素を選択
#symbols = ["H", "Li", "Be", "B", "C", "N", "O", "F"]

# 選び出した元素の２個の組合せ（8元素から2つを選ぶので8C2の組合せ）
Comb_2 = itertools.combinations(symbols, 2) 
#酸化ジスプロシウム（Dy2O3）、酸化マグネシウム（MgO）、酸化マンガン（MnO2）、酸化ケイ素（SiO2）、炭酸バリウム（BaCO3）


# API_KEY="5xospsIpXSGq9sQ3"
# with MPRester(API_KEY) as m:
#     df_COM = pd.DataFrame()
#     #compoundはlist型
#     for elements in Comb_2:
#         print(str(elements[0]+'-'+elements[1]))
#         compound = m.get_data("Ti-Ba-O-"+elements[0]+'-'+elements[1] , data_type='vasp')
#         compound=m.get_data("Ti-Ba-O")
#         df_com = pd.DataFrame(compound)           
#         df_COM = df_COM.append(df_com)
# 
# #結果を保存
# df_COM.to_csv('compound_2.csv')

# In[ ]:


def listConnect(A):
    A=list(A)
    ret=""
    for a in A:
        ret += a+"-"
    return ret[:-1]

Comb_2=itertools.combinations(symbols[3:], 3)
for elements in Comb_2:
    print(listConnect(list(elements)))


# In[ ]:


symbols=["Ti","Ba","O","Dy","Mg","Mn","Si","C"]
Comb_2=itertools.combinations(symbols, 2)
ingredients=["TiBaO3","Dy2O3","MgO","MnO2","SiO2","BaCO3"]

def elementsset(d):
    import pymatgen as mg
    dc=mg.core.Composition(d)
    return [x.name for x in dc.elements]

print([elementsset(d) for d in ingredients])
    
complement_sets=list()
for x in [elementsset(d) for d in ingredients]:
    y=set(symbols)-set(x)
    print(list(y))
    complement_sets.append(list(y))
    
elements_sets=[elementsset(d) for d in ingredients]
print(elements_sets,complement_sets)


# In[ ]:


API_KEY="5xospsIpXSGq9sQ3"
m=MPRester(API_KEY)
print("START")
df_COM = pd.DataFrame()
#compoundはlist型

compound= m.get_data("Ti-Ba-O" , data_type='vasp')
df_com = pd.DataFrame(compound)           
df_COM = df_COM.append(df_com)


def listConnect(A):
    A=list(A)
    ret=""
    for a in A:
        ret += a+"-"
    return ret[:-1]


for a,b in zip(elements_sets,complement_sets):
    for extension in range(1,len(b)):
        Comb_2=itertools.combinations(b, extension)
        for elements in Comb_2:
            toget=listConnect(a)+'-'+listConnect(elements)
            print(toget) 
            compound = m.get_data(toget , data_type='vasp')
            df_com = pd.DataFrame(compound)
            print("size:",len(df_com))
            df_COM = df_COM.append(df_com)
            


# In[ ]:


df_COM.to_csv('compound_2.csv')


# In[ ]:


from pymatgen.core import Composition, Element
from numpy import zeros, mean
trainFile = open("compound_2.csv","r").readlines()


# In[ ]:


#input:pymatgenのCompositionオブジェクト
#output:組成ベクトル
def naiveVectorize(composition):
       vector = zeros((MAX_Z))
       for element in composition:
               #elementは原子。fractionはその原子が組成に含まれる割合
               fraction = composition.get_atomic_fraction(element)
               vector[element.Z - 1] = fraction
       return(vector)


# In[ ]:


for line in trainFile:
       split = str.split(line, ',')
       #material = Composition(split[0])
       #materials.append(material) #化学式
       #naiveFeatures.append(naiveVectorize(material)) #特徴量ベクトル生成
       #bandgaps.append(float(split[1])) #バンドギャップの読み込み


# In[ ]:


bandgaps=[x for x in df_COM["band_gap"]]


# In[ ]:


vectors=list()
materials=list()
MAX_Z=100
for a  in df_COM["full_formula"]:
    print(a)
    vector = zeros((MAX_Z))
    b=Composition(a)
    materials.append(b)
    for element in b:
        fraction = b.get_atomic_fraction(element)
        vector[element.Z - 1] = fraction
    print(vector)
    vectors.append(vector)
    
naiveFeatures=vectors
materials


# In[ ]:


baselineError = mean(abs(mean(bandgaps) - bandgaps))
baselineError


# In[ ]:


from sklearn.model_selection import cross_val_score
from sklearn.model_selection import ShuffleSplit
from sklearn import linear_model, metrics, ensemble

#sklearnのランダムフォレスト回帰
rfr = ensemble.RandomForestRegressor(n_estimators=10)

#交差検証します
cv = ShuffleSplit(n_splits=10, test_size=0.1, random_state=0)

scores_composition = cross_val_score(rfr, naiveFeatures,\
    bandgaps, cv=cv, scoring='neg_mean_absolute_error')

print("Mean Absolute Error by Random Forest with composition data: "\
    + str(round(abs(mean(scores_composition)), 3)) + " eV")


# In[ ]:


rfr.fit(naiveFeatures,bandgaps)


# In[ ]:


bandgaps


# In[ ]:


rfr.predict((naiveFeatures))


# In[ ]:


physicalFeatures = []
ic=0
volumes=[x for x in df_COM["volume"]]
density=[x for x in df_COM["density"]]
for material in materials:
    theseFeatures = []
    fraction = []
    atomicNo = []
    eneg = []
    group = []
    vector = zeros(4*(MAX_Z)+50)
    for element in material:
        vector[element.Z - 1] = material.get_atomic_fraction(element)
        vector[MAX_Z+element.Z - 1] = float(element.Z)
        vector[MAX_Z*2+element.Z - 1] = float(element.X)
        vector[MAX_Z*3+element.Z - 1] = float(element.group)
        vector[MAX_Z*4+1]=volumes[ic]
        vector[MAX_Z*4+1]=density[ic]  
        #fraction.append(material.get_atomic_fraction(element))
        #atomicNo.append(float(element.Z))
        #eneg.append(element.X)
        #group.append(float(element.group))

    #print(material,fraction,atomicNo,eneg,group)

    #mustReverse = False
    #if fraction[1] > fraction[0]:
    #       mustReverse = True

    #for features in [fraction, atomicNo, eneg, group]:
    #       if mustReverse:
    #               features.reverse()
    #theseFeatures.append(fraction[0] / fraction[1])
    #theseFeatures.append(eneg[0] - eneg[1])
    #theseFeatures.append(group[0])
    #theseFeatures.append(group[1])
    physicalFeatures.append(vector)
    ic+=1


# In[ ]:


scores_physical =cross_val_score(rfr, physicalFeatures,\
    bandgaps, cv=cv, scoring='neg_mean_absolute_error')

print("Mean Absolute Error by Random Forest with physical data: "\
    + str(round(abs(mean(scores_physical)), 3)) + " eV")


# In[ ]:


from jarvis.db.figshare import data
d = data('dft_3d') #choose a name of dataset from above
# See available keys
print (d[0].keys())
# Dataset size
print(len(d))

# Visualize an atoms object
from jarvis.core.atoms import Atoms
a = Atoms.from_dict(d[0]['atoms'])
#You can visualize this in VESTA or other similar packages
print(a)

# If pandas framework needed
import pandas as pd
df = pd.DataFrame(d)
print(df)


# In[ ]:


df.columns


# In[ ]:


DielectricConstantAU=1.11265005545e-10 #=F/m
DielactricConstautAir=8.8541878128e-12 #F/m
DielectricConstantAU/DielactricConstautAir


# In[ ]:


for y,x in zip(df.columns,df.iloc[21930]):
    print(y,x)


# In[ ]:


for i in  range(len(df["formula"])):
    if df["formula"][i]=="BaTiO3":
        print("True",i,df["formula"][i],df['mepsx'][i],df['dfpt_piezo_max_dielectric'][i])


# In[ ]:


df["formula"]
vectors=list()
maxeij=list()
materials=list()
ic=0
Zlist=list()
for a,c  in zip(df["formula"],df["dfpt_piezo_max_eij"]):
    if c!="na" and float(c)!=0.0:
        vector = zeros((MAX_Z))
        b=Composition(a)
        materials.append(b)
        vector = zeros((MAX_Z))
        for element in b:
            Zlist.append(element.Z)
            #vector[element.Z - 1] = material.get_atomic_fraction(element)
            #vector[MAX_Z+element.Z - 1] = float(element.Z)
            #vector[MAX_Z*2+element.Z - 1] = float(element.X)
            #vector[MAX_Z*3+element.Z - 1] = float(element.group)
            #vector[MAX_Z*4+1]=df["volumes"][ic]
            vector[MAX_Z-1]=df["density"][ic]  
        for element in b:
            fraction = b.get_atomic_fraction(element)
            vector[element.Z - 1] = fraction
        #print(vector)
        maxeij.append(c)
        vectors.append(vector)
    ic+=1

naiveFeatures=vectors
materials


# In[ ]:


set((Zlist))


# In[ ]:


import numpy as np
min(np.array(maxeij))


# In[ ]:


def 

rfr.predict([naiveFeatures[1]])


# In[ ]:


Zlist


# In[ ]:


from sklearn.model_selection import cross_val_score
from sklearn.model_selection import ShuffleSplit
from sklearn import linear_model, metrics, ensemble

#sklearnのランダムフォレスト回帰
rfr = ensemble.RandomForestRegressor(n_estimators=10)

#交差検証します
cv = ShuffleSplit(n_splits=10, test_size=0.1, random_state=0)

scores_composition = cross_val_score(rfr, naiveFeatures,\
    maxeij, cv=cv, scoring='neg_mean_absolute_error')

print("Mean Absolute Error by Random Forest with composition data: "\
    + str(round(abs(mean(scores_composition)), 3)) + " ")


# In[ ]:


np.max(np.array([naiveFeatures[i][99] for i in range(len(naiveFeatures))]))


# In[ ]:


Zlist=list(set((Zlist)))
Ilist=[0 for _ in range((MAX_Z))]
for i in range(len(Zlist)):
    if Zlist[i]!=0:
        Ilist[i]=1


# In[ ]:


print(Ilist)


# In[ ]:


rfr.fit(naiveFeatures,maxeij)
def objfunc(indivisual):
    X=[0 for _ in range(MAX_Z)]
    for i in range(MAX_Z):
        X[i]=indivisual[i]*Ilist[i]
    X[99]*=15.3
    X=np.array(X)
    Y=rfr.predict([X])
    return Y[0]
        


# In[ ]:


objfunc(naiveFeatures[1])


# In[ ]:


rfr.fit(naiveFeatures,maxeij)


# In[ ]:


rfr.fit(naiveFeatures,maxeij)


# In[ ]:


Y=rfr.predict(naiveFeatures)


# In[ ]:


import matplotlib.pyplot as plt
get_ipython().run_line_magic('matplotlib', 'inline')
x = maxeij
y = Y
plt.scatter(x,y)
plt.xlabel('maxeij')
plt.ylabel('prediction')
plt.title('eij')
plt.show()


# In[ ]:


get_ipython().system('pip install deap')


# In[ ]:


import random

from deap import base
from deap import creator
from deap import tools


# In[ ]:


creator.create("FitnessMax", base.Fitness, weights=(1.0,))
creator.create("Individual", list, fitness=creator.FitnessMax)


# In[ ]:


toolbox = base.Toolbox()
# Attribute generator
toolbox.register("attr_bool", random.randint, 1,10)
# Structure initializers
toolbox.register("individual", tools.initRepeat, creator.Individual, 
    toolbox.attr_bool, 100)
toolbox.register("population", tools.initRepeat, list, toolbox.individual)


# In[ ]:


random.


# In[ ]:


def evalOneMax(individual):
    return sum(individual),

toolbox.register("evaluate", evalOneMax)
toolbox.register("mate", tools.cxTwoPoints)
toolbox.register("mutate", tools.mutFlipBit, indpb=0.05)
toolbox.register("select", tools.selTournament, tournsize=3)


# In[ ]:


main()


# In[ ]:


#個体の各遺伝子を決めるために使用
import random

#DEAPの中にある必要なモジュールをインポート
from deap import base
from deap import creator
from deap import tools
from deap import algorithms

#最小化問題として設定(-1.0で最小化、1.0で最大化問題)
#面食らうかもしれませんが、目的が最小化の場合は以下のように設定します。
creator.create("FitnessMin", base.Fitness, weights=(-1.0,))

#個体の定義（list型と指定しただけで、中身の遺伝子は後で入れる）
#これも面食らうかもしれませんが、個体を準備したと思ってください。
creator.create("Individual", list, fitness=creator.FitnessMin)

#目的関数の定義。必ずreturnの後に,をつける
def obfunc(individual):
    x = individual[0]
    y = individual[1]
    z = individual[2]
    w = individual[3]
    object = (x-0.5)**2 + (y-0.5)**2 + (0.25-z*w)**2
    #(x,y)=(1,2)で最小になるはず。これを遺伝的アルゴリズムで求める
    return object,

rfr.fit(naiveFeatures,maxeij)
def objfunc(individual):
    X=[0 for _ in range(MAX_Z)]
    penalty=0
    notzero=0
    for i in range(MAX_Z):
        X[i]=individual[i]*Ilist[i]
        if X[i]<0:
            penalty+=1
        if X[i]!=0:
            notzero+=1
    if notzero>5:
        penalty+=notzero
    print(notzero)
    X[99]*=15.3
    X=np.array(X)
    Y=rfr.predict([X])
    return penalty+(Y[0]-4)**2,

mymu=[0. for _ in range(MAX_Z)]
mysigma=[0.5 for _ in range(MAX_Z)]

#各種関数の設定を行います
#交叉、選択、突然変異などには、DEAPのToolbox内にある関数を利用
toolbox = base.Toolbox()
#random.uniformの別名をattribute関数として設定。各個体の遺伝子の中身を決める関数(各遺伝子は-50～50のランダムな値)
toolbox.register("attribute", random.uniform, 0,1)
#individualという関数を設定。それぞれの個体に含まれる2個の遺伝子をattributeにより決めるよ、ということ。
toolbox.register("individual", tools.initRepeat, creator.Individual, toolbox.attribute, MAX_Z)
#集団の個体数を設定するための関数を準備
toolbox.register("population", tools.initRepeat, list, toolbox.individual)
#トーナメント方式で次世代に子を残す親を選択（tornsizeは各トーナメントに参加する個体の数）
toolbox.register("select", tools.selTournament, tournsize=5)
#交叉関数の設定。ブレンド交叉という手法を採用
toolbox.register("mate", tools.cxBlend,alpha=0.2)
#突然変異関数の設定。indpbは各遺伝子が突然変異を起こす確率。muとsigmaは変異の平均と標準偏差
toolbox.register("mutate", tools.mutGaussian, mu=mymu, sigma=mysigma, indpb=0.2)
#評価したい関数の設定（目的関数のこと）
toolbox.register("evaluate", objfunc)

#以下でパラメータの設定
#今回は最も単純な遺伝的アルゴリズムの手法を採用

#乱数を固定
random.seed(64)
#何世代まで行うか
NGEN = 50
#集団の個体数
POP = 80
#交叉確率
CXPB = 0.9
#個体が突然変異を起こす確率
MUTPB = 0.1

#集団は80個体という情報の設定
pop = toolbox.population(n=POP)
#集団内の個体それぞれの適応度（目的関数の値）を計算
for individual in pop:
    individual.fitness.values = toolbox.evaluate(individual)
#パレート曲線上の個体(つまり、良い結果の個体)をhofという変数に格納
hof = tools.ParetoFront()

#今回は最も単純なSimple GAという進化戦略を採用
algorithms.eaSimple(pop, toolbox, cxpb=CXPB, mutpb=MUTPB, ngen=NGEN, halloffame=hof)

#最終的な集団(pop)からベストな個体を1体選出する関数
best_ind = tools.selBest(pop, 10)[0]
#結果表示
print("最も良い個体は %sで、そのときの目的関数の値は %s" % (best_ind, best_ind.fitness.values))


# In[ ]:


tools.selBest(pop, 10)


# In[ ]:


rfr.fit(naiveFeatures,maxeij)
MAX_ELEM=4
def objfunc(indivisual):
    elm0=indivisual[0]
    elm1=indivisual[1]
    elm2=indivisual[2]
    elm3=indivisual[3]
    r0=indivisual[4]
    r1=indivisual[5]
    r2=indivisual[6]
    r3=indivisual[7]
    
    tot=r0+r1+r2+r3
    X=[0. for x in range(MAX_Z)]
    X[elm0]=r0/tot
    X[elm1]=r1/tot
    X[elm2]=r2/tot
    X[elm3]=r3/tot
    X[99]*=15.3*individual[8]/92
    X=np.array(X)
    Y=rfr.predict([X])
    return (Y[0]-4)**2,

objfunc([1,35,8,10,12,1,6,7,48])


# In[ ]:


pop = toolbox.population(n=POP)
pop


# In[ ]:


#個体の各遺伝子を決めるために使用
import random

#DEAPの中にある必要なモジュールをインポート
from deap import base
from deap import creator
from deap import tools
from deap import algorithms

#最小化問題として設定(-1.0で最小化、1.0で最大化問題)
#面食らうかもしれませんが、目的が最小化の場合は以下のように設定します。
creator.create("FitnessMin", base.Fitness, weights=(-1.0,))

#個体の定義（list型と指定しただけで、中身の遺伝子は後で入れる）
#これも面食らうかもしれませんが、個体を準備したと思ってください。
creator.create("Individual", list, fitness=creator.FitnessMin)

#目的関数の定義。必ずreturnの後に,をつける
def obfunc(individual):
    x = individual[0]
    y = individual[1]
    z = individual[2]
    w = individual[3]
    object = (x-0.5)**2 + (y-0.5)**2 + (0.25-z*w)**2
    #(x,y)=(1,2)で最小になるはず。これを遺伝的アルゴリズムで求める
    return object,

rfr.fit(naiveFeatures,maxeij)
MAX_ELEM=4
def objfunc(indivisual):
    print(individual)
    
    elm0=int(indivisual[0])
    elm1=int(indivisual[1])
    elm2=int(indivisual[2])
    elm3=int(indivisual[3])
    r0=indivisual[4]
    r1=indivisual[5]
    r2=indivisual[6]
    r3=indivisual[7]
    
    tot=r0+r1+r2+r3
    X=[0. for x in range(MAX_Z)]
    try:
        X[elm0]=r0/tot
        X[elm1]=r1/tot
        X[elm2]=r2/tot
        X[elm3]=r3/tot
        X[99]*=15.3*individual[8]/92
        X=np.array(X)
        Y=rfr.predict([X])
        print(Y)
        return (Y[0]-4)**2,
    except:
        return 100,

mymu=[0. for _ in range(9)]
mysigma=[15 for _ in range(9)]

#各種関数の設定を行います
#交叉、選択、突然変異などには、DEAPのToolbox内にある関数を利用
toolbox = base.Toolbox()
#random.uniformの別名をattribute関数として設定。各個体の遺伝子の中身を決める関数(各遺伝子は-50～50のランダムな値)
toolbox.register("attribute", random.randint, 1,92)
#individualという関数を設定。それぞれの個体に含まれる2個の遺伝子をattributeにより決めるよ、ということ。
toolbox.register("individual", tools.initRepeat, creator.Individual, toolbox.attribute, 9)
#集団の個体数を設定するための関数を準備
toolbox.register("population", tools.initRepeat, list, toolbox.individual)
#トーナメント方式で次世代に子を残す親を選択（tornsizeは各トーナメントに参加する個体の数）
toolbox.register("select", tools.selTournament, tournsize=5)
#交叉関数の設定。ブレンド交叉という手法を採用
toolbox.register("mate", tools.cxBlend,alpha=0.2)
#突然変異関数の設定。indpbは各遺伝子が突然変異を起こす確率。muとsigmaは変異の平均と標準偏差
toolbox.register("mutate", tools.mutGaussian, mu=mymu, sigma=mysigma, indpb=0.2)
#評価したい関数の設定（目的関数のこと）
toolbox.register("evaluate", objfunc)

#以下でパラメータの設定
#今回は最も単純な遺伝的アルゴリズムの手法を採用

#乱数を固定
random.seed(64)
#何世代まで行うか
NGEN = 50
#集団の個体数
POP = 80
#交叉確率
CXPB = 0.9
#個体が突然変異を起こす確率
MUTPB = 0.1

#集団は80個体という情報の設定
pop = toolbox.population(n=POP)
#集団内の個体それぞれの適応度（目的関数の値）を計算
for individual in pop:
    individual.fitness.values = toolbox.evaluate(individual)
#パレート曲線上の個体(つまり、良い結果の個体)をhofという変数に格納
hof = tools.ParetoFront()

#今回は最も単純なSimple GAという進化戦略を採用
algorithms.eaSimple(pop, toolbox, cxpb=CXPB, mutpb=MUTPB, ngen=NGEN, halloffame=hof)

#最終的な集団(pop)からベストな個体を1体選出する関数
best_ind = tools.selBest(pop, 10)[0]
#結果表示
print("最も良い個体は %sで、そのときの目的関数の値は %s" % (best_ind, best_ind.fitness.values))


# In[ ]:


# -*- coding: utf-8 -*-
import array
import random
import json

import numpy as np
import matplotlib.pyplot as plt

from math import sqrt

from deap import algorithms
from deap import base
from deap import benchmarks
from deap.benchmarks.tools import diversity, convergence, hypervolume
from deap import creator
from deap import tools

creator.create("FitnessMin", base.Fitness, weights=(-1.0, -1.0))
creator.create("Individual", array.array, typecode='d', fitness=creator.FitnessMin)

toolbox = base.Toolbox()

BOUND_LOW, BOUND_UP = 0.0, 1.0

NDIM = 30

def uniform(low, up, size=None):
    try:
        return [random.uniform(a, b) for a, b in zip(low, up)]
    except TypeError:
        return [random.uniform(a, b) for a, b in zip([low] * size, [up] * size)]

toolbox.register("attr_float", uniform, BOUND_LOW, BOUND_UP, NDIM)
toolbox.register("individual", tools.initIterate, creator.Individual, toolbox.attr_float)
toolbox.register("population", tools.initRepeat, list, toolbox.individual)

toolbox.register("evaluate", benchmarks.zdt1)
toolbox.register("mate", tools.cxSimulatedBinaryBounded, low=BOUND_LOW, up=BOUND_UP, eta=20.0)
toolbox.register("mutate", tools.mutPolynomialBounded, low=BOUND_LOW, up=BOUND_UP, eta=20.0, indpb=1.0/NDIM)
toolbox.register("select", tools.selNSGA2)

def main(seed=None):
    random.seed(seed)

    NGEN = 250
    MU = 100
    CXPB = 0.9

    stats = tools.Statistics(lambda ind: ind.fitness.values)
    stats.register("min", np.min, axis=0)
    stats.register("max", np.max, axis=0)
    
    logbook = tools.Logbook()
    logbook.header = "gen", "evals", "min", "max"
    
    pop = toolbox.population(n=MU)
    pop_ini = pop[:]
    
    invalid_ind = [ind for ind in pop if not ind.fitness.valid]
    fitnesses = toolbox.map(toolbox.evaluate, invalid_ind)
    for ind, fit in zip(invalid_ind, fitnesses):
        ind.fitness.values = fit

    pop = toolbox.select(pop, len(pop))
    
    record = stats.compile(pop)
    logbook.record(gen=0, evals=len(invalid_ind), **record)
    print(logbook.stream)

    for gen in range(1, NGEN):

        offspring = tools.selTournamentDCD(pop, len(pop))
        offspring = [toolbox.clone(ind) for ind in offspring]
        
        for ind1, ind2 in zip(offspring[::2], offspring[1::2]):
            if random.random() <= CXPB:
                toolbox.mate(ind1, ind2)
            
            toolbox.mutate(ind1)
            toolbox.mutate(ind2)
            del ind1.fitness.values, ind2.fitness.values
        
        invalid_ind = [ind for ind in offspring if not ind.fitness.valid]
        fitnesses = toolbox.map(toolbox.evaluate, invalid_ind)
        for ind, fit in zip(invalid_ind, fitnesses):
            ind.fitness.values = fit

        pop = toolbox.select(pop + offspring, MU)
        record = stats.compile(pop)
        logbook.record(gen=gen, evals=len(invalid_ind), **record)
        print(logbook.stream)

    print("Final population hypervolume is %f" % hypervolume(pop, [11.0, 11.0]))

    return pop, pop_ini, logbook
        
if __name__ == "__main__":
    pop, pop_ini, stats = main(64)

    fitnesses_ini = np.array([list(pop_ini[i].fitness.values) for i in range(len(pop_ini))])
    fitnesses = np.array([list(pop[i].fitness.values) for i in range(len(pop))])

    plt.plot(fitnesses_ini[:,0], fitnesses_ini[:,1], "b.", label="Initial")
    plt.plot(fitnesses[:,0], fitnesses[:,1], "r.", label="Optimized" )
    plt.legend(loc="upper right")
    plt.title("fitnesses")
    plt.xlabel("f1")
    plt.ylabel("f2")
    plt.grid(True)
    plt.savefig("fitnesses.png", dpi=300)



==> name2.tex <==
Computer Programs Python (Machine learning and Neural Network)

matminer
A property-oriented design strategy for high performance copper alloys via machine learning
https://www.nature.com/articles/s41524-019-0227-7

xenonpy
"Predicting Materials Properties with Little Data Using Shotgun Transfer Learning"
https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6813555/

ElemNet
"ElemNet: Deep Learning the Chemistry of Materials From Only Elemental Composition"
https://www.nature.com/articles/s41598-018-35934-y


Descriptor
https://github.com/EXJUSTICE/LISICON_NASICON_IonicConductivity_Classification

Maybe we have to prepare the dataset (with various composition ration) in a table, as is attached to EXJUSTICE.


Database

The Open Quantum Materials Database (OQMD): assessing the accuracy of DFT formation energies
https://www.nature.com/articles/npjcompumats201510/#:~:text=The%20Open%20Quantum%20Materials%20Database%20%28OQMD%29%20is%20a,%28ICSD%29%20and%20decorations%20of%20commonly%20occurring%20crystal%20structures.

Materials Project
https://legacy.materialsproject.org/


